A Calculus for Flow-Limited Authorization

Real-world applications routinely make authorization decisions based on dynamic computation. Reasoning about dynamically computed authority is challenging. Integrity of the system might be compromised if attackers can improperly influence the authorizing computation. Confidentiality can also be compromised by authorization, since authorization decisions are often based on sensitive data such as membership lists and passwords. Previous formal models for authorization do not fully address the security implications of permitting trust relationships to change, which limits their ability to reason about authority that derives from dynamic computation. Our goal is an approach to constructing dynamic authorization mechanisms that do not violate confidentiality or integrity. The Flow-Limited Authorization Calculus (FLAC) is a simple, expressive model for reasoning about dynamic authorization as well as an information flow control language for securely implementing various authorization mechanisms. FLAC combines the insights of two previous models: it extends the Dependency Core Calculus with features made possible by the Flow-Limited Authorization Model. FLAC provides strong end-to-end information security guarantees even for programs that incorporate and implement rich dynamic authorization mechanisms. These guarantees include noninterference and robust declassification, which prevent attackers from influencing information disclosures in unauthorized ways. We prove these security properties formally for all FLAC programs and explore the expressiveness of FLAC with several examples.

==> flacproofs.tex <==

\subsection{FLAC Syntax }

\begin{figure}[!h]
\[
\small
\begin{array}{rcl}
\multicolumn{3}{l}{ n \in \mathcal N \text{  (primitive principals)}} \\
\multicolumn{3}{l}{ x \in \mathcal V \text{  (variable names)}} \\
\\
p,ℓ,\pc &::=&  n \sep \top \sep \bot \sep \confid{p} \sep \integ{p} \sep p ∧ p\sep p ∨ p \\[0.4em] %
τ &::=&  \aftype{p}{p} \sep \voidtype \sep \sumtype{τ}{τ} \sep \prodtype{τ}{τ} \\[0.4em]  
  & &\sep  \func{τ}{\pc}{τ} \sep \says{ℓ}{τ} \sep X \sep \tfunc{X}{τ} \\[0.4em]  
v &::=&  () \sep \pair{v}{v} \sep \delexp{p}{p} \sep \return{ℓ}{v} \\[0.4em]  
  &&  \sep \inji{v}  \sep \lamc{x}{τ}{\pc}{e}  \sep \tlam{X}{\pc}{e} \\[0.4em]  
  && \sep \where{v}{v}  \\[0.4em] 
e &::=&  x \sep v \sep  e~e \sep \pair{e}{e} \sep \return{ℓ}{e} \\[0.4em]
   && \sep eτ \sep \proji{e} \sep \inji{e} \\[0.4em]  
   && \sep \casexp{v}{x}{e}{e} \\[0.4em]  
   && \sep \bind{x}{e}{e} \sep \assert{e}{e} \\[0.4em] 
\end{array}
\hfill
\]
\caption{FLAC syntax}
\label{fig:flacsyntax}
\end{figure}
\begin{figure}
\[
\small
\begin{array}{rcl}
E & ::= &  [\cdot] \sep E~e \sep v~E \sep \pair{E}{e} \sep \pair{v}{E} \sep \proji{E} \sep \inji{E} \\[0.4em]  
  && \sep \return{ℓ}{E} \sep \bind{x}{E}{e} \\[0.4em]
   && \sep Eτ \sep \assume{E}{e} \sep \casexp{E}{x}{e}{e} \\[0.4em]  
\end{array}
\hfill
\]
\caption{FLAC Evaluation Contexts}
\label{fig:eval}
\end{figure}

\autoref{fig:flacexpsem} presents the FLAC evaluation rules.

\begin{figure*}[t]
{\footnotesize
\begin{flalign*}
& \boxed{
	e \stepsone e'
} &
\end{flalign*}
\begin{mathpar}
\ferule*{E-App}{}{(\lamc{x}{τ}{\pc}{e})~v}{\subst{e}{x}{v}}{}

\ferule*{E-TApp}{}{(\tlam{X}{\pc}{e})~τ}{\subst{e}{X}{τ}}{}

\ferule*{E-UnPair}{}{\proj{i}{\tuple{v_1}{v_2}}}{v_i}{}

\ferule*{E-Case1}{}{(\casexp{(\ione{v})}{x}{e_1}{e_2}) }{\subst{e_1}{x}{v}}{}

\ferule*{E-Case2}{}{(\casexp{(\itwo{v})}{x}{e_1}{e_2}) }{ \subst{e_2}{x}{v}}{}

\ferule*{E-BindM}{}{\bind{x}{\return{ℓ}{v}}{e}}{\subst{e}{x}{v}}{}

\ferule{E-Assume}{}{\assume{\delexp{p}{q}}{e}}{\where{e}{\delexp{p}{q}}}{}

\ferule{E-Eval}{e \stepsone e'}{E[e]}{E[e']}{}

\ferule{W-App}{}{(\where{v}{\delexp{a}{b}})~v'}{\where{(v~v')}{\delexp{a}{b}}}{}

\ferule{W-TApp}{}{(\where{v}{\delexp{a}{b}})~s}{\where{(v~s)}{\delexp{a}{b}}}{}

\ferule{W-UnPair}{}{\proj{i}{(\where{\pair{v_1}{v_2}}{\delexp{a}{b}})}}{\where{(\proj{i}{\pair{v_1}{v_2}})}{\delexp{a}{b}}}{}

\ferule{W-Case}{}{(\casexp{(\where{v}{\delexp{a}{b}})}{x}{e_1}{e_2})}{\where{(\casexp{v}{x}{e_1}{e_2})}{\delexp{a}{b}}}{}

\ferule{W-UnitM}{}{\return{\ell}{\where{v}{\delexp{a}{b}}}}{\where{\return{\ell}{v}}{\delexp{a}{b}}}{}

\ferule{W-BindM}{}{\bind{x}{(\where{v}{\delexp{a}{b}})}{e}}{\where{(\bind{x}{v}{e})}{\delexp{a}{b}}}{}

	\ferule{W-Assume}{}{\assume{(\where{\delexp{p}{q}}{\delexp{a}{b}})}{e}}{\where{(\assume{\delexp{p}{q}}{e})}{\delexp{a}{b}}}{}

\end{mathpar}
}
\caption{FLAC Semantics}
\label{fig:flacexpsem}
\end{figure*}

\autoref{fig:flactypesys} presents modified FLAC type system.
The rules differ from the original FLAC formulation with the invariant that any term that is well typed in the original type system is also well-typed in this modified type system.

\begin{figure*}
\begin{mathpar}
	\Rule{Var}{}
	{\fexp{\delegcontext}{\varcontext,x\ty τ}{\pc}{x}{τ}}

	\Rule{Unit}{}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\void}{\voidtype}}

	\Rule{Del}{}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}}}

	\Rule{Lam}
	{\fexp{\delegcontext}{\varcontext,x\ty τ₁}{\pc'}{e}{τ_2}}
	{\fexp{\delegcontext}{\varcontext}{pc}{\lamc{x}{τ₁}{\pc'}{e}}{\func{τ_1}{\pc'}{τ_2}}}

	\Rule{App}
	{
	\fexp{\delegcontext}{\varcontext}{\pc}{e}{\func{τ_1}{\pc'}{τ_2}} \\\\
	\fexp{\delegcontext}{\varcontext}{\pc}{e'}{τ_1} \\
	\rflowjudge{\delegcontext;\pubtrust;\pc'}{\pc}{\pc'}
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{e~e'}{τ_2}}

	\Rule{TLam}
	{
		\fexp{\delegcontext}{\varcontext, X}{\pc'}{e}{\tau}
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\tlam{X}{\pc'}{e}}{\tfunc{X}{\tau}}}

	\Rule{TApp}
	{
	\fexp{\delegcontext}{\varcontext}{\pc}{e}{\tfunc{X}{\tau}} \\
	\rflowjudge{\delegcontext;\pubtrust;\pc'}{\pc}{\pc'}
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{e~\tau'}{τ[X \mapsto \tau']}}

	\Rule{Pair}
	{
	\fexp{\delegcontext}{\varcontext,~x:τ_1}{pc}{e_1}{τ_1} \\
	\fexp{\delegcontext}{\varcontext,~x:τ_2}{pc}{e_2}{τ_2}
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\pair{e_1}{e_2}}{\prodtype{τ_1}{τ_2}}}
        
	\Rule{UnPair}
	{
		\fexp{\delegcontext}{\varcontext,~x:τ_1}{pc}{e}{\prodtype{τ_1}{τ_2}} 
	}
	{\fexp{\delegcontext}{\varcontext}{pc}{\proj{i}{e}}{τ_i}}
        
	\Rule{Inj}
	{ \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau_i}
	}
	{  \fexp{\delegcontext}{\varcontext}{\pc}{\inj{i}{e}}{\sumtype{\tau_1}{\tau_2}}}

	\Rule{Case}
	{
	\fexp{\delegcontext}{\varcontext}{\pc}{e}{τ_1 + τ_2} \\
	\protjudge{\delegcontext;\pubtrust;\ell}{\pc \sqcup \ell}{\tau} \\
	\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc}{\ell} \\
	\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc \sqcup \ell }{e_1}{τ} \\
	\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc \sqcup \ell}{e_2}{τ} \\
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\casexp{e}{x}{e_1}{e_2}}{τ}}
        
	\Rule{UnitM}
	{\fexpPGTpc{e}{\tau} 
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\return{\ell}{e}}{\says{\ell}{\tau}}}

	\Rule{BindM}
	{ \fexpPGTpc{e}{\says{\ell}{\tau'}}\\
		\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc \sqcup \ell \sqcup \ell'}{e'}{\tau} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau}
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\bind{x}{e}{e'}}{\tau}}

	\Rule{Assume}
	{ \fexpPGTpc{e}{\aftype{p}{q}} \\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \\
		\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc \sqcup \ell \sqcup \ell'}{e'}{\tau} 
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\assume{e}{e'}}{\tau}}
        
	\Rule{Where}
	{ 
		\fexp{\delegcontext}{\varcontext}{\pc}{v}{{p}\actsfor{q}} \\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \\
		\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{e}{\tau} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau} 
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\where{e}{v}}{\tau}}
\end{mathpar}
\caption{FLAC new typing rules}
\label{fig:flactypesys}
\end{figure*}

Figure~\ref{fig:tprotrules} shows type protection rules. \ruleref{P-Del} is not present in the original FLAC formulation.

\begin{figure*}
\begin{mathpar}
	\Rule{R-Static}
	{\stafjudge{\L}{p}{q}}
	{\rafjudge{\delegcontext;\pc; \ell}{p}{q}} 

	\Rule{R-Assume}
	{
		\delexpl{p}{q}{\ell'} \in \delegcontext \\
		\rflowjudge{\delegcontext;\pc \sqcup \ell'; \ell}{\ell'}{\ell \wedge \voice{q}} \\
		\rafjudge{\delegcontext;\pc; \ell}{\pc}{\voice{q}} \\
		\rafjudge{\delegcontext;\pc; \ell}{\voice{\confid{p}}}{\voice{\confid{q}}} 
	}
	{\rafjudge{\delegcontext;\pc; \ell}{p}{q}} 

	\Rule{R-ConjR}
	{ \rafjudge{\delegcontext;\pc; \ell}{p}{q_1} \\
		\rafjudge{\delegcontext;\pc; \ell}{p}{q_2} 
	} 
	{\rafjudge{\delegcontext;\pc; \ell}{p}{q_1 \wedge q_2}} 

	\Rule{R-DisjL}
	{
		\rafjudge{\delegcontext;\pc; \ell}{p_1}{q} \\
		\rafjudge{\delegcontext;\pc; \ell}{p_2}{q} 
	} 
	{\rafjudge{\delegcontext;\pc; \ell}{p_1 \vee p_2}{q}} 

	\Rule{R-Trans}
	{
		\rafjudge{\delegcontext;\pc; \ell}{p}{q} \\
		\rafjudge{\delegcontext;\pc; \ell}{q}{r} \\
		\rafjudge{\delegcontext;\pc; \ell}{\pc}{\voice{\confid{r}}}
	} 
	{\rafjudge{\delegcontext;\pc; \ell}{p}{r}} 

	\Rule{R-Weaken}
	{\rafjudge{\delegcontext;\pc'; \ell'}{p}{q} \\ 
		\rflowjudge{\delegcontext;\pc ; \ell}{\ell'}{\ell} \\
		\rflowjudge{\delegcontext;\pc ; \ell}{\pc}{\pc'} 
	}
	{\rafjudge{\delegcontext;\pc; \ell}{p}{q}} 
\end{mathpar}
\caption{FLAC Robust Assumption}
\label{fig:robassume}
\end{figure*}

\begin{figure*}
\begin{mathpar}
	\Rule{P-Unit}{}
	{\protjudge{\delegcontext;\pc;\ell}{\ell'}{\voidtype}} 

	\Rule{P-Pair}
	{\protjudge{\delegcontext;\pc;\ell}{\ell'}{\tau_1} \\
		\protjudge{\delegcontext;\pc;\ell}{\ell'}{\tau_2} 
	}
	{\protjudge{\delegcontext;\pc;\ell}{\ell'}{\prodtype{\tau_1}{\tau_2}}} 

	\Rule{P-Fun}
	{ \rflowjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\pc'}  \\
	  \rflowjudge{\delegcontext;\pubtrust;\pc'}{\ell}{\pc'}  \\
	\protjudge{\delegcontext;\pc;\ell}{\ell'}{\tau_2} 
	}
	{\protjudge{\delegcontext;\pc; \ell}{\ell'}{\func{\tau_1}{\pc'}{\tau_2}}} 

	\Rule{P-TFun}
	{ \rflowjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\pc'}  \\
	  \rflowjudge{\delegcontext;\pubtrust;\pc'}{\ell}{\pc'}  \\
	\protjudge{\delegcontext;\pc;\ell}{\ell'}{\tau} 
	}
	{\protjudge{\delegcontext;\pc;\ell}{\ell'}{\tfunc{X}{\tau}}}

	\Rule{P-Lbl1}
	{\protjudge{\delegcontext;\pc; \ell}{\ell'}{\tau} 
	}
	{\protjudge{\delegcontext;\pc; \ell}{\ell'}{\says{\ell''}{\tau}}}

	\Rule{P-Lbl2}
	{\rflowjudge{\delegcontext;\pc;\ell}{\ell'}{\ell''} 
	}
	{\protjudge{\delegcontext;\pc;\ell}{\ell'}{\says{\ell''}{\tau}}}

	\Rule{P-Del}{}
	{\protjudge{\delegcontext;\pc; \ell }{\ell'}{\aftype{a}{b}}} \\
\end{mathpar}
\caption{FLAC type protection rules}
\label{fig:tprotrules}
\end{figure*}

\subsection{FLAC Proofs}

\begin{lemma}[FLAC implies FLAM]
	Let $\delegcontext = \mathcal{H}(c)$. If
	$\rafjudge{\delegcontext;\pc;\ell}{p}{q}$, then
	$\rafjudge{\mathcal{H};c;\pc;\ell}{p}{q}$.
\end{lemma}
\begin{proof}
	Proof is by induction on the derivation of the robust assumption
	$\rafjudge{\delegcontext;\pc;\ell}{p}{q}$. Interesting case is \ruleref{R-Assume}. 
	\begin{description}
		\item[Case R-Assume:] From the premises, we have, that

	\begin{align}
		\delexpl{p}{q}{\ell \wedge \voice{q}} \in \delegcontext \label{eq:1}\\
		\protjudge{\delegcontext;\pc;\ell}{\pc \sqcup \ell}{\tau} \label{eq:2} \\
		\rafjudge{\delegcontext;\pc; \ell}{\pc}{\voice{q}} \label{eq:3}\\
		\rafjudge{\delegcontext;\pc; \ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:4}
	\end{align}

	From \eqref{eq:1} and \ruleref{Del}, we have that
	\[
		\afjudge{\mathcal{H};c;\pc;\ell'}{p}{q}
	\]

	From \eqref{eq:2} and  \ruleref[Weaken], we get that
	$\afjudge{\mathcal{H};c;\pc;\ell \wedge \voice{q}}{p}{q}$.
	From the \eqref{eq:3}, \eqref{eq:4} and \ruleref{R-Lift} we thus have
	$\rafjudge{\mathcal{H};c;\pc;\ell}{p}{q}$.

\item[Case R-Static:] Since $\stafjudge*{p}{q}$, we have that
	\[
		\mathcal{H};c; \confid{\bot} \wedge \integ{\top}; \ell  \vdash p~\actsfor~q
	\]
	From FLAM \ruleref{R-Static}, we thus have,
	$\rafjudge{\mathcal{H};c;\pc;\ell}{p}{q}$.

	\item[Case R-ConjR:] Trivial.
	\item[Case R-DisjL:] Trivial.
	\item[Case R-Trans:] Trivial.
	\item[Case R-Weaken:] Trivial.
	\end{description}
	
\end{proof}

\begin{figure*}
\begin{mathpar}
	\ferule*{B-Step}{{e_i}\stepsone{e_i'} \\ e_j = e_j' \\ \{i, j\} = \{1, 2\}}{\bracket{e_1}{e_2}}{\bracket{e_1'}{e_2'}}{}

	\ferule*{B-App}{}{\bracket{\lamc{x}{\tau_1}{\pc_1}{e_1}}{\lamc{x}{\tau_2}{\pc_2}{e_2}}~v}{\bracket{e_1[x \mapsto \outproj{v}{1}]}{e_2[x \mapsto \outproj{v}{2}]}}{}

	\ferule*{B-TApp}{}{\bracket{\tlam{X}{\pc}{e_1}}{\tlam{X}{\pc}{e_2}}~\tau}{\bracket{e_1[X \mapsto \tau]}{e_2[X \mapsto \tau]}}{}


	\ferule*{B-UnPair}{}{\proj{i}{\bracket{\pair{v_{11}}{v_{12}}}{\pair{v_{11}}{v_{22}}}}}{\bracket{v_{1i}}{v_{2i}}}{}

	\ferule*{B-BindM1}{\ell_1 \ne \ell_2}{\bind{x}{\bracket{\return{\ell_1}{v_1}}{\return{\ell_2}{v_2}}}{e}}{\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}e[x \mapsto {v_2}]}}{}

	\ferule*{B-BindM2}{}{\bind{x}{\bracket{\return{\ell}{v_1}}{\return{\ell}{v_2}}}{e}}{e[x \mapsto \bracket{v_1}{v_2}]}{}

	\ferule*{B-BindM3}{}{\bind{x}{\bracket{\return{\ell}{v_1}}{\return{\ell}{v_2}}}{e}}{\bracket{e[x \mapsto {v_1}]}{e[x \mapsto {v_2}]}}{}

	\ferule*{B-Case}{}{\casexp{\bracket{\inj{i}{v_1}}{\inj{j}{v_2}}}{x}{e_1}{e_2}}{\bracket{\outproj{e_i}{1}[x \mapsto {v_1}]}{\outproj{e_j}{2}[x \mapsto {v_2}]}}{}

\end{mathpar}
	\caption{Evaluation extensions}
	\label{fig:beval}
\end{figure*}

\begin{figure*}
\begin{align*}
	\outproj{e}{i} = \begin{cases} 
		v_i &\mbox{ if } e = \bracket{v_1}{v_2} \\
		x &\mbox{ if } e = x \\
		\outproj{e}{i}~\outproj{e'}{i} &\mbox{ if } e = e~e' \\
		\pair{\outproj{e_1}{i}}{\outproj{e_2}{i}} &\mbox{ if } e = \pair{e_1}{e_2} \\
		\return{\ell}{\outproj{e}{i}} &\mbox{ if } e = \return{\ell}{e} \\
		{\outproj{e}{i}}~\tau &\mbox{ if } e = e~\tau \\
		{\proj{j}{\outproj{e}{i}}} &\mbox{ if } e = \proj{j}{e} \\
		{\casexp{\outproj{v}{i}}{x}{\outproj{e_1}{i}}{\outproj{e_2}{i}}} &\mbox{ if } e = \casexp{v}{x}{e_1}{e_2} \\
		{\bind{x}{\outproj{e}{i}}{\outproj{e'}{i}}} &\mbox{ if } e = \bind{x}{e}{e'} \\
		{\assume{\outproj{e}{i}}{\outproj{e'}{i}}} &\mbox{ if } e = \assume{e}{e'} \\
		e_i &\mbox{ if } e = \bracket{e_1}{e_2}  \\
	\end{cases}
\end{align*}
	\caption{Projection for bracketed expressions}
	\label{fig:projection}
\end{figure*}

Figure~\ref{fig:beval} shows evaluation extensions.
Nesting of bracketed expressions isn't allowed.

Figure~\ref{fig:projection} defines projection.
Typing extensions shown in Figure~\ref{fig:typeext}.
\begin{figure*}
\begin{mathpar}
	\Rule{Bracket}
	{
		\fexp{\delegcontext}{\varcontext}{\pc'}{e_1}{\tau} \\
		\fexp{\delegcontext}{\varcontext}{\pc'}{e_2}{\tau} \\
	\rflowjudge{\delegcontext;\pubtrust;\ell}{(\ell \sqcup \ell' \sqcup H^\pi \sqcup \pc)}{{\pc'}} \\
		\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\tau} \\
		\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \\
		\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} 
	}
	{\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1}{e_2}}{\tau}}
\end{mathpar}
	\caption{Typing Extensions}
	\label{fig:typeext}
\end{figure*}

\begin{lemma}[Soundness]\label{lemma:sound}
	If $e \stepsone e'$ then $\outproj{e}{i} \stepsone \outproj{e'}{i}$ for $i = \{1, 2\}$.
\end{lemma}
\begin{proof}
			\todo{in progress}
	Proof is by induction on the derivation $e \stepsto e'$. The only interesting cases are \ruleref{B-Step}, \ruleref{B-App} and \ruleref{B-Case}. 
	\begin{description}
		\item[Case B-Step:] Since $\bracket{e_1}{e_2} \stepsone \bracket{{e'}_1}{{e'}_2}$, we have that $e_i \stepsone {e'}_i$. Since $e_i = \outproj{e}{i}$and ${e'}_i = \outproj{e'}{i}$, we have that    $\outproj{e}{i} \stepsone \outproj{e'}{i}$.
		\item[Case B-App:]
		\item[Case B-TApp:]
		\item[Case B-Proj:]
		\item[Case B-BindM1:]
		\item[Case B-BindM2:]
		\item[Case B-BindM3:]
		\item[Case B-Case:]
	\end{description}
\end{proof}

\begin{lemma}[Stuck Expressions]\label{lemma:stuck}
 If $e$ gets stuck then $\outproj{e}{i}$ is stuck for some $i =\{1,2\}$.
\end{lemma}
\begin{proof}
We prove by induction on the structure of $e$ that if $e$ gets stuck then $\outproj{e}{i}$ is stuck for some $i =\{1,2\}$.
	\begin{description}
		\item[Case $v$:] By assumption, $e$ is not a value.
		\item[Case $x$:] No reduction for a variable. Hence \outproj{x}{i} is stuck as well.
		\item[Case $e~e'$:] Since \ruleref{B-App} and \ruleref{E-App} are not applicable, it follows that $e$ is not of the form $\bracket{\lamc{x}{\tau}{\pc'}{e_1}}{\lamc{x}{\tau}{\pc'}{e_2}}$ or$\lamc{x}{\tau}{\pc}{e}$. Thus \outproj{e}{i} is stuck as well.
		\item[Case $\return{\ell}{e}$:] Since $e$ is stuck, applying induction hypothesis it follows that $\outproj{e}{i}$ is also stuck and so $\outproj{\return{\ell}{e}}{i}$ is also stuck.
		\item[Case $\proj{j}{e}$, $\inj{j}{e}$:] Similar to the above case.
		\item[Case $e~\tau$:] Since \ruleref{B-TApp} and \ruleref{E-TApp} are not applicable, it follows that $e$ is not of the form $\bracket{v_1}{v_2}$ or $\tlam{X}{\pc}{e}$. Thus $\outproj{e}{i}~\tau$ is stuck as well.
		\item[Case $\casexp{v}{x}{e_1}{e_2}$:] Since \ruleref{B-Case} and \ruleref{E-Case} are not applicable, it follows that $e$ is not of the form $\bracket{v_1}{v_2}$ or $\inj{j}{e}$. It follows that 
			
			$\outproj{\casexp{v}{x}{e_1}{e_2}}{i}$ is also stuck. 
		\item[Case $\bind{x}{e}{e'}$:] Similar to the above case.
		\item[Case $\assume{e}{e'}$:] Similar to the above case.
		\item[Case Bracket:] $e = \bracket{e_1}{e_2}$. The only way this gets stuck is if both $e_1$ and $e_2$ get stuck. This is a contradiction.
	\end{description}
\end{proof}

\begin{lemma}[Completeness]\label{lemma:complete}
	If $\outproj{e}{1} \stepsto v_1$ and $\outproj{e}{2} \stepsto v_2$ then
	there exists a $v$ such that $e \stepsto v$. 
\end{lemma}
\begin{proof}
	Assume that $e$ diverges. Then by Lemma~\ref{lemma:sound}, $\outproj{e}{i}$ diverges for some $i =\{1,2\}$. This is a contradiction. Thus $e$ does not diverge.
	Now assume that $e$ gets stuck. 
 By Lemma~\ref{lemma:stuck}, if $e$ gets stuck then $\outproj{e}{i}$ is stuck for some $i =\{1,2\}$. This is a contradiction.
	Thus $e$ does not get stuck. Hence there exists a $v$ such that $e \stepsto v$. 
\end{proof}

\begin{lemma}[Projection Preserves Types]\label{lemma:proj}
	If \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau}, then
	 \fexp{\delegcontext}{\varcontext}{\pc}{\outproj{e}{i}}{\tau} for $i = \{1, 2\}$.
\end{lemma}
\begin{proof}
	Proof is by induction on the typing derivation.
\end{proof}
\begin{lemma}[Values]\label{lemma:values}
	If  \fexp{\delegcontext}{\varcontext}{\pc}{v}{\tau} then
 \fexp{\delegcontext}{\varcontext}{\pc'}{v}{\tau} for any $\pc'$. 
\end{lemma}
\begin{proof}
	Proof is by induction on the structure of $\fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau}$. 
	\begin{description}
		\item[Var:] Not a value.
		\item[Lam:] Trivial.
		\item[App:] Not a value.
		\item[TLam:] From \ruleref{TLam}, we have that $\tlam{X}{\pc'}{e}$ can be typed under any $\pc$. 
		\item[TApp:] Not a value.
		\item[Pair:] Applying induction to the premises we have
			$\fexp{\delegcontext}{\varcontext}{\pc'}{v_i}{\tau_i}$ for $i = \{1, 2\}$. Hence 
			$\fexp{\delegcontext}{\varcontext}{\pc'}{\pair{v_1}{v_2}}{\prodtype{\tau_1}{\tau_2}}$ 
		\item[Unpair:] Not a value.
		\item[Inj:] Applying induction to the premise, we have
	$\fexp{\delegcontext}{\varcontext}{\pc'}{v}{\tau_2}$. Hence, 
	$\fexp{\delegcontext}{\varcontext}{\pc'}{v}{\sumtype{\tau_1}{\tau_2}}$ 
		\item[Case:] Not a value.
		\item[BindM:] Not a value.
		\item[Assume:] Not a value.
		\item[Where:] Follows from applying induction to the premises.
	\end{description}
\end{proof}

\begin{lemma}[Robust Assumption] \label{lemma:robassumption}
	If
	$\rafjudge{\delegcontext;\pc;\pc}{\pc}{\voice{b}}$, then
	$\rafjudge{\delegcontext, \delexpl{a}{b}{\pc'};\pc;\pc}{\pc}{\voice{b}}$ for any $a, b, \pc'$.
\end{lemma}


\begin{lemma}[Robust Protection] \label{lemma:robprotect}
	If
	$\protjudge{\delegcontext;\pc; \ell}{\pc}{\tau}$,  
	then
	$\protjudge{\delegcontext, \delexpl{a}{b}{\pc'};\pc; \ell}{\pc}{\tau}$ for any $a, b, \pc'$. 
\end{lemma}


\begin{lemma}[\delegcontext Weakening]\label{lemma:piweaken}
	If  \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau} then
	\fexp{\delegcontext, \delexpl{p}{q}{\pc'}}{\varcontext}{\pc}{e}{\tau} for any $p, q, pc' \in \L$.
\end{lemma}
\begin{proof}
	Proof is by induction on the derivation of the typing judgment.
	\begin{description}
		\item[Case Var: ] Trivial.
		\item[Case Unit: ] Trivial.
		\item[Case Del: ] Trivial.
		\item[Case Lam: ] Trivial.
		\item[Case App: ] Trivial.
		\item[Case TApp: ] Trivial.
		\item[Case Pair: ] Trivial.
		\item[Case UnPair: ] Trivial.
		\item[Case Inj: ] Trivial.
		\item[Case Case: ] Trivial.
		\item[Case UnitM: ] Trivial.
		\item[Case BindM: ] Trivial.
		\item[Case Assume: ] Given 
	$\fexp{\delegcontext}{\varcontext}{\pc}{\assume{e}{e'}}{\tau}$. From the premises,
\begin{align}
	\fexpPGTpc{e}{\aftype{a}{b}} \label{eq:piwassume1} \\
	\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{b}} \label{eq:piwassume2}\\
	\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{a}}}{\voice{\confid{b}}} \label{eq:piwassume3} \\
	\fexp{\delegcontext, \delexpl{a}{b}{\pc \sqcup \ell}}{\varcontext}{\pc \sqcup \ell \sqcup \ell'}{e'}{\tau} \label{eq:piwassume4}\\
	\protjudge{\delegcontext;\pubtrust; \ell'}{\pc\sqcup \ell \sqcup \ell'}{\tau} \label{eq:piwassume5}
\end{align}
Applying inductive step to \eqref{eq:piwassume1} and \eqref{eq:piwassume4}, we have 
$\fexp{\delegcontext, \delexpl{a}{b}{\pc \sqcup \ell},\delexpl{p}{q}{pc'}}{\varcontext}{\pc}{e'}{\tau}$ and 

\fexp{\delegcontext, \delexpl{p}{q}{\pc'}}{\varcontext}{\pc}{e}{\aftype{a}{b}}.
From Lemma~\ref{lemma:robassumption}, we have 
$\rafjudge{\delegcontext, \delexpl{p}{q}{\pc'} ;\pubtrust;\ell}{\pc}{\voice{b}}$ and
$\rafjudge{\delegcontext,\delexpl{p}{q}{\pc'} ;\pubtrust;\ell}{\voice{\confid{a}}}{\voice{\confid{b}}}$.
Applying Lemma ~\ref{lemma:robprotect} to \eqref{eq:piwassume5}, we have

\protjudge{\delegcontext, \delexpl{p}{q}{\pc'}; \pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau}. 
Thus, we have all the premises required to derive
$\fexp{\delegcontext, \delexpl{p}{q}{\pc}}{\varcontext}{pc}{\assume{e}{e'}}{\tau}$. 

		\item[Case Where: ] Similar to the proof of case \ruleref{Assume}.
		\item[Case Bracket:] Applying induction to the premises of \ruleref{Bracket} gives us that $\fexp{\delegcontext, \delexpl{a}{b}{\ell}}{\varcontext}{\pc}{\bracket{e_1}{e_2}}{\tau}$.
	\end{description}
\end{proof}


\begin{lemma}[Flow Transitivity]\label{lemma:flowtrans}
If 
$\rflowjudge{\delegcontext;\pubtrust; \pc}{p}{q}$ and
$\rflowjudge{\delegcontext;\pubtrust; \pc}{q}{r}$ then
$\rflowjudge{\delegcontext;\pubtrust; \pc}{r}{s}$.
\end{lemma}
\begin{proof}
	Follows from \ruleref{R-Trans}.
\end{proof}

\begin{lemma}[Protection]\label{lemma:flowprot}
	If 
	$\rflowjudge{\delegcontext;\pubtrust; \ell}{\ell''}{\ell'}$ and 
	$\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\tau}$ then
	$\protjudge{\delegcontext; \pubtrust; \ell}{\ell''}{\tau}$.
\end{lemma}
\begin{proof}
 Proof is by induction on the protection judgment.
	\begin{description}
		\item[Case P-Unit:] Trivial
		\item[Case P-Del:] Trivial
		\item[Case P-Pair:] Applying inductive hypothesis to the premises, we have 
			$\protjudge{\delegcontext; \pubtrust; \ell}{\ell''}{\prodtype{\tau_1}{\tau_2}}$.
		\item[Case P-Fun:] From \ruleref{P-Fun}, we have
		\begin{align}
			\rflowjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\pc'} \label{eq:fpfun1} \\
	  	 \rflowjudge{\delegcontext;\pubtrust;\pc'}{\ell}{\pc'} \label{eq:fpfun2} \\
		 \protjudge{\delegcontext;\pc;\ell}{\ell'}{\tau_2} \label{eq:fpfun3}
		\end{align}
			Applying inductive hypothesis to \eqref{eq:fpfun3}, we have 
		 $\protjudge{\delegcontext;\pc;\ell}{\ell''}{\tau_2}$ 
			Applying \ruleref{R-Trans} to $\rflowjudge{\delegcontext;\pubtrust; \ell}{\ell''}{\ell'}$ and \eqref{eq:fpfun1}, we have 
			\rflowjudge{\delegcontext;\pubtrust;\ell}{\ell''}{\pc'}.

			We now have all premises required to prove
	${\protjudge{\delegcontext;\pc; \ell}{\ell''}{\func{\tau_1}{\pc'}{\tau_2}}}$ 

\item[Case P-TFun:] Similar to above case
\item[Case P-Lbl1:] Applying inductive hypothesis to the premise, we have
	$\protjudge{\delegcontext;\pc; \ell}{\ell''}{\says{\ell'''}{\tau}}$. 
\item[Case P-Lbl2:] Applying \ruleref{R-Trans} to  $\rflowjudge{\delegcontext;\pubtrust; \ell}{\ell''}{\ell'}$ and the premise, we have
$\rflowjudge{\delegcontext;\pubtrust; \ell}{\ell''}{\ell'''}$. And so, 
	$\protjudge{\delegcontext;\pc; \ell}{\ell''}{\says{\ell'''}{\tau}}$. 
	\end{description}
\end{proof}


\begin{lemma}[Substitution]\label{lemma:subst}
If \fexp{\delegcontext}{\varcontext, x:\tau'}{\pc}{e}{\tau} 
and	\fexp{\delegcontext}{\varcontext}{\pc}{v}{\tau'}, then 
\fexp{\delegcontext}{\varcontext}{\pc}{e[x \mapsto v]}{\tau}. 
\end{lemma}
\begin{proof}
	Proof is by the induction on the structure of the expression $e$.
\end{proof}

\begin{lemma}[Type Substitution Preserves Well-Typedness]\label{lemma:typesubst}
	Let $\tau'$ be well-formed in $\varcontext, X, \varcontext'$.
If \fexp{\delegcontext}{\varcontext, X, \varcontext'}{\pc}{e}{\tau} 
	then \fexp{\delegcontext}{\varcontext, \varcontext'[X \mapsto \tau']}{\pc}{e[X \mapsto \tau']}{\tau [X \mapsto \tau']}. 
\end{lemma}
\begin{proof}
	Proof is by the induction on the typing derivation $\fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau}$. 
	\begin{description}
		\item[Case Var:] Depending on whether $\tau$ uses $X$ two cases arise.
			Either \fexp{\delegcontext}{\varcontext,x:\tau, X, \varcontext'}{\pc}{x}{\tau} or \fexp{\delegcontext}{\varcontext,X, x:\tau, \varcontext'}{\pc}{x}{\tau}. 
			In the former case,
			since $\varcontext, x: \tau$ does not use $X$, we have that
			$\tau [X \mapsto \tau']$ is same as $\tau$.

			In the latter case, we have that \fexp{\delegcontext}{\varcontext,X, x:\tau[X \mapsto \tau'], \varcontext'[X \mapsto \tau']}{\pc}{x}{\tau[X \mapsto \tau']}. 
		\item[Case Unit:] Trivial.
		\item[Case Del:] Trivial.
		\item[Case Lam:] Given $\fexp{\delegcontext}{\varcontext, X, \varcontext'}{\pc}{\lamc{x}{\tau_1}{\pc'}{e}}{\func{\tau_1}{\pc'}{\tau_2}}$. 
			From \ruleref{Lam} $\fexp{\delegcontext}{\varcontext, X, \varcontext', x:\tau_1}{\pc'}{e}{\tau_2}$. 
			Applying induction hypothesis to the premise, we have
			$\fexp{\delegcontext}{\varcontext, \varcontext'[X \mapsto \tau'], x:\tau_1[X \mapsto \tau']}{\pc'}{e[X \mapsto \tau']}{\tau_2 [X \mapsto \tau']}$. 
			From \ruleref{Lam}, we thus have $\fexp{\delegcontext}{\varcontext, \varcontext'[X \mapsto \tau']}{\pc}{\lamc{x}{\tau_1}{\pc'}{e[X \mapsto \tau']}}{\func{\tau_1[X \mapsto \tau']}{\pc'}{\tau_2[X \mapsto \tau']}}$. 

		\item[Case App:] Given $\fexp{\delegcontext}{\varcontext, X, \varcontext'}{\pc}{e~e'}{\tau_2}$. Applying induction hypothesis to the premises, we have 
			\begin{align}
				\fexp{\delegcontext}{\varcontext, X, \varcontext'[X \mapsto \tau']}{\pc}{e[X \mapsto \tau']}{\func{\tau_1[X \mapsto \tau']}{\pc'}{\tau_2[X \mapsto \tau']}} \\
				\fexp{\delegcontext}{\varcontext, X, \varcontext'[X \mapsto \tau']}{\pc}{e'[X \mapsto \tau']}{\tau_1[X \mapsto \tau']}
			\end{align}

			From \ruleref{App}, we thus have
			$\fexp{\delegcontext}{\varcontext, X, \varcontext'[X \mapsto \tau']}{\pc}{e[X \mapsto \tau']~e'[X \mapsto \tau']}{\tau_2[X \mapsto \tau']}$

		\item[Case TLam:] Given
			$\fexp{\delegcontext}{\varcontext, X, \varcontext'}{\pc}{\tlam{Y}{\pc'}{e}}{\tfuncpc{Y}{\pc'}{\tau}}$. Applying induction hypothesis to the premise of \ruleref{TLam} we have
			\[
				\fexp{\delegcontext}{\varcontext, (\varcontext', Y)[X \mapsto \tau']}{\pc'}{e[X \mapsto \tau']}{\tau[X \mapsto \tau']}
			\]
			So from \ruleref{TLam}, we have
			$$\fexp{\delegcontext}{\varcontext, \varcontext'[X \mapsto \tau']}{\pc}{\tlam{Y}{\pc'}{e[X \mapsto \tau']}}{\tfuncpc{Y}{\pc'}{\tau[ X \mapsto \tau'}}$$.

		\item[Case TApp:] Given
			$\fexp{\delegcontext}{\varcontext, X, \varcontext'}{\pc}{e~\tau''}{\tau[Y \mapsto \tau'']}$. Applying induction hypothesis to the premises of \ruleref{TApp}, we have $\fexp{\delegcontext}{\varcontext, X, \varcontext'[X \mapsto \tau']}{\pc}{e[X \mapsto \tau']}{\tfuncpc{Y}{\pc'}{\tau[X \mapsto \tau']}}$. From \ruleref{TApp}, we thus have
			$\fexp{\delegcontext}{\varcontext, \varcontext'[X \mapsto \tau']}{\pc}{(e[X \mapsto \tau'])~\tau''[X \mapsto \tau']}{\tau[X \mapsto \tau'][Y \mapsto \tau'']}$
		\item[Case Pair:] Straight forward application of induction hypothesis to the premises.
		\item[Case UnPair:] Straight forward application of induction hypothesis to the premises.
		\item[Case Inj:] Straight forward application of induction hypothesis to the premises.
		\item[Case Case:] Straight forward application of induction hypothesis to the premises.
		\item[Case UnitM:] Straight forward application of induction hypothesis to the premises.
		\item[Case BindM:] Straight forward application of induction hypothesis to the premises.
		\item[Case Assume:] Straight forward application of induction hypothesis to the premises.
		\item[Case Where:] Straight forward application of induction hypothesis to the premises.
	\end{description}

\end{proof}

\begin{lemma}[Type Substitution Preserves Protection]\label{lemma:substprot}
	Let $\tau'$ be well-formed in $\varcontext$. Also let $X$ be a type variable that is lexically present in the type $\tau$. 
	If \protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\tau} then
	\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\tau [ X \mapsto \tau']}
\end{lemma}
\begin{proof}
	Proof is by induction on the structure of the types.
	\begin{description}
		\item[Case $\voidtype$ :] Given $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\voidtype}$. Since $\voidtype [X \mapsto \tau']$ is $\voidtype$, we have that
	\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\voidtype[ X \mapsto \tau']}.

\item[Case $\aftype{p}{q}$: ] Given $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\aftype{p}{q}}$. Since $\aftype{p}{q} [X \mapsto \tau']$ is $\aftype{p}{q}$, we have that
	\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\aftype{p}{q}[ X \mapsto \tau']}.

		\item[Case $X$:] Since $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{X}$ doesn't hold, this is an invalid case.
\item[Case $\sumtype{\tau_1}{\tau_2}$:] Since $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\sumtype{\tau_1}{\tau_2}}$ doesn't hold, this is an invalid case.

\item[Case $\prodtype{\tau_1}{\tau_2}$:] Given $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\prodtype{\tau_1}{\tau_2}}$. Applying induction hypothesis to the premises of \ruleref{P-Pair}, we have $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\tau_1[X \mapsto \tau']}$ and $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\tau_2[X \mapsto \tau']}$. From \ruleref{P-Pair}, we thus have $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\prodtype{\tau_1[X \mapsto \tau']}{\tau_2[X \mapsto \tau']}}$.


\item[Case $\func{\tau_1}{\pc}{\tau_2}$:] Applying induction to the premises of \ruleref{P-Fun}, we get $\protjudge{\delegcontext;\pubtrust;\ell}{\ell'}{\func{\tau_1[X \mapsto \tau']}{\pc}{\tau_2[X \mapsto \tau'}}$.

\item[Case $\says{\ell}{\tau}$:] Given $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\says{\ell''}{\tau}}$. 
	
	If $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\tau}$ then applying induction to the premises of \ruleref{P-Lbl1}, we get that $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\says{\ell''}{\tau[X \mapsto \tau'}}$.

			If $\rflowjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\ell''}$ then from \ruleref{P-Lbl2} we have $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\says{\ell''}{\tau[X \mapsto \tau'}}$.
		\item[Case $\tfuncpc{X}{\pc}{\tau}$:] Applying induction hypothesis to the premises of \ruleref{P-TFun}, we get that $\protjudge{\delegcontext; \pubtrust; \ell}{\ell'}{\tfuncpc{X}{\pc}{\tau [X \mapsto \tau']}}$.
	\end{description}

	Hence proved.
\end{proof}

\begin{lemma}[PC Reduction]\label{lemma:pcred}
	For all $\pc, \pc'$, such that 
	\rflowjudge{\delegcontext;\pubtrust; \pc}{\pc'}{\pc}
	if \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau} 
	then 
	\fexp{\delegcontext}{\varcontext}{\pc'}{\outproj{e}{i}}{\tau} for $i \in \{1, 2\}$.
\end{lemma}
\begin{proof} 
	Proof is by induction on the derivation of the typing judgment.
	\begin{description}
		\item[Case Var: ] Trivial.
		\item[Case Unit: ] Trivial.
		\item[Case Del: ] Trivial.
		\item[Case Lam: ] Trivial.
		\item[Case App: ]
			Given,
	${\fexp{\delegcontext}{\varcontext}{\pc}{e~e'}{τ_2}}$.
	From \ruleref{App}, we have
	\begin{align}
		\fexp{\delegcontext}{\varcontext}{\pc}{e}{\func{τ_1}{\pc''}{τ_2}} \label{eq:pcredapp1} \\
		\fexp{\delegcontext}{\varcontext}{\pc}{e'}{τ_1} \label{eq:pcredapp2}\\
		\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc}{\pc''} \label{eq:pcredapp3}
	\end{align}
	
	Applying inductive hypothesis to \eqref{eq:pcredapp1} and \eqref{eq:pcredapp2}, we have
		$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{\func{τ_1}{\pc''}{τ_2}}$  and 
		$\fexp{\delegcontext}{\varcontext}{\pc'}{e'}{τ_1}$. 

		We need to show that
		\[
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}
		\]
		Using \eqref{eq:pcredapp3} we weaken the result label of
	$\rflowjudge{\delegcontext;\privuntrust; \pc}{\pc'}{\pc}$ to get
			$\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}$
		Combining, we have all the premises for \ruleref{App} and thus
	$${\fexp{\delegcontext}{\varcontext}{\pc'}{e~e'}{τ_2}}$$
		\item[Case TApp: ] 
			Given
	${\fexp{\delegcontext}{\varcontext}{\pc}{e~τ'}{τ}}$.
	From \ruleref{TApp}, we have
	\begin{align}
		\fexp{\delegcontext}{\varcontext}{\pc}{e}{\tfuncpc{X}{\pc''}{τ}} \label{eq:pcredtapp1} \\
		\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc}{\pc''} \label{eq:pcredtapp2}
	\end{align}
	
	Applying inductive hypothesis to \eqref{eq:pcredtapp1}, we have 
		$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{\tfuncpc{X}{\pc''}{τ}}$.
		We still need to show that
		\[
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}
		\]
		Using \eqref{eq:pcredtapp2} we weaken the result label of
	$\rflowjudge{\delegcontext;\privuntrust; \pc}{\pc'}{\pc}$ to get
			$\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}$
		Combining, we have all the premises for \ruleref{TApp} and thus
	$${\fexp{\delegcontext}{\varcontext}{\pc'}{e~τ'}{τ}}$$
		\item[Case Pair: ] Given 
	${\fexp{\delegcontext}{\varcontext}{\pc}{\pair{e_1}{e_2}}{\prodtype{τ_1}{τ_2}}}$.
	Applying inductive hypothesis to the premises of \ruleref{Pair}, we have 
	$\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc'}{e_1}{τ_1}$ and $ \fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc'}{e_2}{τ_2}$. 
	From \ruleref{Pair} we thus have,
	${\fexp{\delegcontext}{\varcontext}{\pc'}{\pair{e_1}{e_2}}{\prodtype{τ_1}{τ_2}}}$
        
		\item[Case UnPair: ] Given 
			${\fexp{\delegcontext}{\varcontext}{\pc'}{\proj{i}{e_i}}{τ_i}}$
	Applying inductive hypothesis to the premises of \ruleref{UnPair}, we have 
	$\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc'}{e}{\prodtype{τ_1}{τ_2}}$.
	From \ruleref{UnPair} we thus have,

	${\fexp{\delegcontext}{\varcontext}{\pc'}{\proj{i}{e}}{τ_i}}$.
        
		\item[Case Inj: ] Trivial.
		\item[Case Case: ] 
			Given 
	$\fexp{\delegcontext}{\varcontext}{\pc}{\casexp{e}{x}{e_1}{e_2}}{τ}$.
	From the premises,
			\begin{align}
				\fexp{\delegcontext}{\varcontext}{\pc}{e}{τ_1 + τ_2} \label{eq:pcredcase1}\\
				\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc \sqcup \ell }{e_1}{τ} \label{eq:pcredcase2}\\
				\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc \sqcup \ell}{e_2}{τ} \label{eq:pcredcase3} \\ 
				\protjudge{\delegcontext;\pubtrust;\ell}{\pc \sqcup \ell}{\tau} \label{eq:pcredcase4}\\
				\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc}{\ell} \label{eq:pcredcase5}
	\end{align}	
        
	Applying inductive hypothesis to the premises \eqref{eq:pcredcase1}, \eqref{eq:pcredcase2} and \eqref{eq:pcredcase3}, we have
	$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{τ_1 + τ_2}$
			$\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc' \sqcup \ell }{e_1}{τ}$ and 
				$\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc' \sqcup \ell}{e_2}{τ}$ 
				From \eqref{eq:pcredcase4}, we have
				$\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\tau}$. Using \eqref{eq:pcredcase4} and \ruleref{R-Weaken}, we weaken the result label of 
				$\rflowjudge{\delegcontext;\pubtrust; \pc}{\pc'}{\pc}$ to get 
$\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc'}{\pc}$.
Applying flow transitivity (\autoref{lemma:flowtrans}), we get
$\protjudge{\delegcontext;\pubtrust;\ell}{\pc'}{\tau}$ and so 
$\protjudge{\delegcontext;\pubtrust;\ell}{\pc' \sqcup \ell}{\tau}$.
Similarly, we get
$\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc'}{\ell}$. Combining, we have all the premises for \ruleref{Case} and so,
	$\fexp{\delegcontext}{\varcontext}{\pc'}{\casexp{e}{x}{e_1}{e_2}}{τ}$.

	\item[Case UnitM: ] Trivial.
		\item[Case BindM: ] 
			Given,
			${\fexp{\delegcontext}{\varcontext}{pc}{\bind{x}{e}{e'}}{τ}}$.
	From \ruleref{BindM}, we have
	\begin{align}
		\fexp{\delegcontext}{\varcontext}{\pc}{e}{\says{\ell}{\tau'}} \label{eq:pcredbind1} \\
		\fexp{\delegcontext}{\varcontext}{\pc \sqcup \ell \sqcup \ell' }{e'}{τ} \label{eq:pcredbind2}\\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell' }{\tau} \label{eq:pcredbind3} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:pcredbind4}
	\end{align}
	
	Applying inductive hypothesis to \eqref{eq:pcredbind1}, we have 
	$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{\says{\ell}{\tau'}}$  and 
	Since $\rflowjudge{\delegcontext; \pubtrust; \pc \sqcup \ell \sqcup \ell'}{\pc' \sqcup \ell \sqcup \ell'}{\pc \sqcup \ell \sqcup \ell'}$,
	applying inductive hypothesis to \eqref{eq:pcredbind2}, we have
		$\fexp{\delegcontext}{\varcontext}{\pc' \sqcup \ell \sqcup \ell'}{e'}{τ}$.

		From $\rflowjudge{\delegcontext; \pubtrust; \pc}{\pc'}{\pc}$
		and \eqref{eq:pcredbind4}, using \ruleref{R-Weaken}, we have
		\begin{equation}
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\pc} \label{eq:pcredbind5}
		\end{equation}

		From $ \protjudge{\delegcontext;\pubtrust; \ell''}{\pc}{\tau}$ and using \ruleref{R-Trans}, we have 
$ \protjudge{\delegcontext;\pubtrust; \ell'}{\pc'}{\tau}$. So,
		$ \protjudge{\delegcontext;\pubtrust; \ell'}{\pc' \sqcup \ell \sqcup \ell' }{\tau}$. 

		Similarly, using \ruleref{R-Trans} on \eqref{eq:pcredbind4} and \eqref{eq:pcredbind5}, we have

		$\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc'}{\ell'}$
		Combining, we have all the premises for \ruleref{BindM} and thus
		$${\fexp{\delegcontext}{\varcontext}{\pc'}{\bind{x}{e}{e'}}{τ}}$$

		\item[Case Assume: ] 
			Given,
			${\fexp{\delegcontext}{\varcontext}{\pc}{\assume{e}{e'}}{τ}}$.
	From \ruleref{Assume}, we have
	\begin{align}
		\fexpPGTpc{e}{\aftype{p}{q}} \label{eq:pcredassume1}\\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:pcredassume2}\\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:pcredassume3}\\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau} \label{eq:pcredassume4}\\
		\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc \sqcup \ell \sqcup \ell'}{e'}{\tau} \label{eq:pcredassume5} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:pcredassume6}\\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:pcredassume7}
	\end{align}
	
	Applying inductive hypothesis to \eqref{eq:pcredassume1}, we have 
	$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{\aftype{p}{q}}$. 
	Since $\rflowjudge{\delegcontext; \pubtrust; \pc \sqcup \ell \sqcup \ell'}{\pc' \sqcup \ell \sqcup \ell'}{\pc \sqcup \ell \sqcup \ell'}$,
	applying inductive hypothesis to \eqref{eq:pcredassume5}, we have
		$\fexp{\delegcontext}{\varcontext}{\pc' \sqcup \ell \sqcup \ell'}{e'}{τ}$.

		Invoking \ruleref{R-Weaken} 
		using $\rflowjudge{\delegcontext; \pubtrust; \pc}{\pc'}{\pc}$
		and \eqref{eq:pcredassume7}, we have 
		\begin{equation}
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\pc} \label{eq:pcredassume8}
		\end{equation}
			From \eqref{eq:pcredassume4}, we have 
			$\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau}$.
		Invoking Lemma~\ref{lemma:flowprot} on $\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau}$ and \eqref{eq:pcredassume8}, we have 
		$ \protjudge{\delegcontext;\pubtrust; \ell'}{\pc'}{\tau}$. 
		So,
		$ \protjudge{\delegcontext;\pubtrust; \ell'}{\pc' \sqcup \ell \sqcup \ell' }{\tau}$. 

		\medskip
		From $\rflowjudge{\delegcontext; \pubtrust; \pc}{\pc'}{\pc}$
		and \eqref{eq:pcredassume6}, using \ruleref{R-Weaken}, we have
		\begin{equation}
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc'}{\pc}\label{eq:pcredassume9}
		\end{equation}
		From \eqref{eq:pcredassume9}, we have  
		\begin{equation}
			\rafjudge{\delegcontext;\pubtrust; \ell}{\pc'}{\pc} \label{eq:pcredassume10}
		\end{equation}
		Using \ruleref{R-Trans} on \eqref{eq:pcredassume2} and \eqref{eq:pcredasseum10}, we have $ \rafjudge{\delegcontext;\pubtrust; \ell}{\pc'}{\voice{q}}$. 
		Invoking Lemma~\ref{lemma:flowtrans} on \eqref{eq:pcredassume8} and \eqref{eq:pcredassume6}, 
		we have $\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc'}{\ell}$.
		Similarly, from \eqref{eq:pcredassume9} and \eqref{eq:pcredassume7}, we have $\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\ell'}$.
		Combining, we have all the premises for \ruleref{Assume} and thus
		$${\fexp{\delegcontext}{\varcontext}{\pc'}{\assume{e}{e'}}{τ}}$$

		\item[Case Where: ] 
			Given,
			${\fexp{\delegcontext}{\varcontext}{\pc}{\where{e}{v}}{τ}}$.
	From \ruleref{Where}, we have
	\begin{align}
		\fexpPGTpc{v}{\aftype{p}{q}} \label{eq:pcredwhere1}\\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:pcredwhere2}\\
		\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:pcredwhere3}\\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\tau} \label{eq:pcredwhere4}\\
		\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc }{e}{\tau} \label{eq:pcredwhere5} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:pcredwhere6}\\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:pcredwhere7}
	\end{align}
	
	
	Applying inductive hypothesis to \eqref{eq:pcredwhere1} and \ref{eq:pcredwhere5}, we have 
	$\fexp{\delegcontext}{\varcontext}{\pc'}{v}{\aftype{p}{q}}$ and 
		$\fexp{\delegcontext}{\varcontext}{\pc'}{e}{τ}$.
		From $\rflowjudge{\delegcontext; \pubtrust; \pc}{\pc'}{\pc}$
		and \eqref{eq:pcredwhere7}, using \ruleref{R-Weaken}, we have
		\begin{equation}
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\pc} \label{eq:pcredwhere8}
		\end{equation}
		From \eqref{eq:pcredwhere4}, we have 
		$\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau}$.
		Using \ruleref{R-Trans}, we have 
$ \protjudge{\delegcontext;\pubtrust; \ell'}{\pc'}{\tau}$. 

		\medskip
		From $\rflowjudge{\delegcontext; \pubtrust; \pc}{\pc'}{\pc}$
		and \eqref{eq:pcredwhere6}, using \ruleref{R-Weaken}, we have
		\begin{equation}
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc'}{\pc} \label{eq:pcredwhere9}
		\end{equation}
		Using \ruleref{R-Trans} on \eqref{eq:pcredwhere2} and above judgment, we have 

		$ \rafjudge{\delegcontext;\pubtrust; \ell}{\pc'}{\voice{q}}$. 
		Using \ruleref{R-Trans} on \eqref{eq:pcredwhere8} and \eqref{eq:pcredwhere6}, we have $\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc'}{\ell}$.
		Similarly, \ruleref{R-Trans} on \eqref{eq:pcredwhere9} and \eqref{eq:pcredwhere7}, we have $\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\ell'}$.
		Combining, we have all the premises for \ruleref{Where} and thus
		$${\fexp{\delegcontext}{\varcontext}{\pc'}{\where{e}{v}}{τ}}$$

		\item[Case Bracket:] Given 
			$\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1}{e_2}}{τ}$. We have to prove that 
			$\fexp{\delegcontext}{\varcontext}{\pc'}{\bracket{e_1}{e_2}}{τ}$.
			From \ruleref{Bracket}, we have
			\begin{align}
				\fexp{\delegcontext}{\varcontext}{\pc''}{e_1}{\tau} \label{eq:pcredbracket1} \\
				\fexp{\delegcontext}{\varcontext}{\pc''}{e_2}{\tau} \label{eq:pcredbracket2} \\
				\rflowjudge{\delegcontext;\pubtrust;\ell}{(H^\pi \sqcup \pc \sqcup \ell \sqcup \ell')}{\pc''} \label{eq:pcredbracket3}\\
				\protjudge{\delegcontext; \pubtrust; \ell'}{\pc''}{\tau} \label{eq:pcredbracket4} \\
				\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \label{eq:pcredbracket5} \\
				\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} \label{eq:pcredbracket6}
			\end{align}
			From \eqref{eq:pcredbracket5}, using \ruleref{R-Weaken} on \rflowjudge{\delegcontext;\pubtrust;\pc}{\pc'}{\pc}, we have
\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc'}{\pc}. 
From \eqref{eq:pcredbracket3} and \ruleref{R-Trans}, we have
				$\rflowjudge{\delegcontext;\pubtrust;\ell}{(H^\pi \sqcup \pc' \sqcup \ell \sqcup \ell')^\pi}{\pc''}$.
				Similarly, from \eqref{eq:pcredbracket5} and \ruleref{R-Trans}, we have
\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc'}{\ell}. Likewise, we have 
\rflowjudge{\delegcontext;\pubtrust;\ell'}{\pc'}{\ell'}.

Combining, we have all the premises for \ruleref{Bracket} and thus we have,
			$\fexp{\delegcontext}{\varcontext}{\pc'}{\bracket{e_1}{e_2}}{τ}$.
	\end{description}

	Completes the proof.
\end{proof}


\begin{lemma}[Subject Reduction]\label{lemma:subred}
	If  \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau} and
	$e \rightarrow e''$, then $\exists~e'$ such that 
	\begin{enumerate}
		\item $e \rightarrow e'$;
		\item \fexp{\delegcontext}{\varcontext}{\pc}{e'}{\tau} and 
		\item $\outproj{e'}{i} = \outproj{e''}{i}$ for $ i = \{1, 2\}$.
	\end{enumerate}
\end{lemma}
\begin{proof}

	Proof is by induction on the evaluation derivation. For all cases except \ruleref{B-BindM1} and \ruleref{B-BindM2}, we have that $e'' = e'$.
	\begin{description}

		\item[Case E-App:] Given $e = (\lamc{x}{\tau_1}{\pc'}{e})~v$ and $e' = e[x \mapsto v]$. Also $\fexp{\delegcontext}{\varcontext}{\pc}{\lamc{x}{\pc'}{e}~v}{\tau_2}$.
			From the premises of \ruleref{App}, we have:
			\begin{align}
				\fexp{\delegcontext}{\varcontext}{\pc}{\lamc{x}{\tau_1}{\pc'}{e}}{\func{τ_1}{\pc'}{τ_2}} \label{eq:subapp1}\\
				\fexp{\delegcontext}{\varcontext}{\pc}{v}{τ_1} \label{eq:subapp2} \\
				\rflowjudge{\delegcontext;\pubtrust;\pc'}{\pc}{\pc'} \label{eq:subapp3}
			\end{align}
			From \eqref{eq:subapp1}, we further have that $\fexp{\delegcontext}{\varcontext, x:\tau_1}{\pc'}{e}{\tau_2}$.
			Since \eqref{eq:subapp3} holds, we can now apply PC reduction (Lemma \autoref{lemma:pcred}) to get $\fexp{\delegcontext}{\varcontext, x:\tau_1}{\pc}{e}{\tau_2}$.
			Applying substitution preservation (Lemma~\ref{lemma:subst}) using \eqref{eq:subapp2},  we have $\fexp{\delegcontext}{\varcontext}{\pc}{e[x \mapsto v]}{\tau_2}$.
         
	\item[Case E-TApp:]Given $e = (\tlam{X}{\pc'}{e})~τ'$ and $e' = e[X \mapsto τ']$. 
		Also $\fexp{\delegcontext}{\varcontext}{\pc}{\tlam{X}{\pc'}{e}~τ'}{\tau [X \mapsto \tau']}$.
			From the premises of \ruleref{TApp}, we have:
			\begin{align}
				\fexp{\delegcontext}{\varcontext}{\pc}{\tlam{X}{\pc'}{e}}{\tfuncpc{X}{\pc'}{τ}} \label{eq:subtapp1}\\
				\rflowjudge{\delegcontext;\pubtrust;\pc'}{\pc}{\pc'} \label{eq:subtapp2}
			\end{align}
			From \ruleref{TLam} and \eqref{eq:subtapp1}, we further have that $\fexp{\delegcontext}{\varcontext, X}{\pc'}{e}{\tau}$.
			Since \eqref{eq:subtapp2} holds, we can now apply PC reduction (Lemma~\ref{lemma:pcred}) to get $\fexp{\delegcontext}{\varcontext, X}{\pc}{e}{\tau}$.
			From type substitution (Lemma~\ref{lemma:typesubst}), we have $$\fexp{\delegcontext}{\varcontext}{\pc}{e[X \mapsto \tau']}{\tau[X \mapsto \tau']}$$.

		\item[Case E-UnPair:] Given $e = \proj{i}{\tuple{v_1}{v_2}}$ and $e' = v_i$. Using Lemma~\ref{lemma:values}, we have that $\fexp{\delegcontext}{\varcontext}{\pc}{v_i}{\tau_i}$.

	\item[Case E-Case:]
		Given $e = {\casexp{\inj{i}{v}}{x}{e_1}{e_2}}$ and $e' = e_i[x \mapsto v]$  
		and that 

		${\fexp{\delegcontext}{\varcontext}{\pc}{\casexp{\inj{i}{v}}{x}{e_1}{e_2}}{τ}}$.
	
	\begin{align}
		\fexp{\delegcontext}{\varcontext}{\pc}{\inj{i}{v}}{τ_1 + τ_2} \label{eq:subcase1}\\
		\protjudge{\delegcontext;\pubtrust;\ell}{\pc \sqcup \ell}{\tau} \label{eq:subcase2}\\
		\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc}{\ell} \label{eq:subcase3}\\
		\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc \sqcup \ell }{e_1}{τ} \label{eq:subcase4}\\
		\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc \sqcup \ell}{e_2}{τ} \label{eq:subcase5} 
	\end{align}

			Since $\rflowjudge{\delegcontext; \pubtrust; \pc \sqcup \ell}{\pc}{\pc \sqcup \ell}$, we can apply PC reduction (Lemma \autoref{lemma:pcred}) to \eqref{eq:subcase4} and \eqref{eq:subcase5} to get
		$\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc}{e_1}{τ}$ and 
		$\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc}{e_2}{τ}$.
		From \eqref{eq:subcase1} and \ruleref{Inj}, we have
		$\fexp{\delegcontext}{\varcontext}{\pc}{v}{τ_i}$.
		Applying Lemma ~\autoref{lemma:subst}, we have that
		$\fexp{\delegcontext}{\varcontext}{\pc}{e_i [x \mapsto v]}{τ}$  for $i = \{1,2\}$.

	\item[Case E-BindM:]
		Given $e = \bind{x}{\return{\ell'}{v}}{e}$ and $e' = e[x \mapsto v]$. Also,  
		$\fexp{\delegcontext}{\varcontext}{\pc}{\bind{x}{\return{\ell'}{v}}{e}}{\tau}$.
	\begin{align}
		\fexpPGTpc{\return{\ell'}{v}}{\says{\ell'}{\tau'}} \label{eq:subbind1}\\
		\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc \sqcup \ell' \sqcup \ell''}{e}{\tau} \label{eq:subbind2} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell''}{\pc}{\ell''} \label{eq:subbind3} \\
		\protjudge{\delegcontext;\pubtrust; \ell''}{\pc \sqcup \ell' \sqcup \ell''}{\tau} \label{eq:subbind4}
	\end{align}

	From \eqref{eq:subbind1} and \ruleref{UnitM}, we have that $\fexp{\delegcontext}{\varcontext}{\pc}{v}{\tau'}$.

			Since $\rflowjudge{\delegcontext;\pubtrust; \pc \sqcup \ell' \sqcup \ell''}{\pc}{ \pc \sqcup \ell \sqcup \ell'}$, applying PC reduction (Lemma~\autoref{lemma:pcred}) to \eqref{eq:subbind2} gives us
		$\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc}{e}{\tau}$.
		Applying Lemma~\ref{lemma:subst} (substitution) to the above judgment, we get
		$\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc}{e[x \mapsto v]}{\tau}$.
	\item[Case E-Assume:]
		Given $e = \assume{\delexp{p}{q}}{e}$ and $e' = \where{e}{\delexp{p}{q}}$. Also,
		${\fexp{\delegcontext}{\varcontext}{\pc}{\assume{\delexp{p}{q}}{e}}{\tau}}$.
		\begin{align}
			\fexpPGTpc{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:subassume1}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:subassume2} \\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:subassume3}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau} \label{eq:subassume4}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:subassume5}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:subassume6}\\
			\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc \sqcup \ell \sqcup \ell'}{e}{\tau} \label{eq:subassume7}
	\end{align}
        
	We have all the premises required for typing \ruleref{Where} and hence
	${\fexp{\delegcontext}{\varcontext}{\pc}{\where{e}{\delexp{p}{q}}}{\tau}}$.

\item[Case E-Eval:] Given $e = E[e]$ and $e' = E[e']$. Also $\fexp{\delegcontext}{\varcontext}{\pc}{E[e]}{\tau}$. This implies that
$\fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau'}$ and
$\fexp{\delegcontext}{\varcontext}{\pc}{E}{\tau}$ (\todo{???}).
	Applying induction to the premise, we have
$\fexp{\delegcontext}{\varcontext}{\pc}{e'}{\tau'}$ and so
$\fexp{\delegcontext}{\varcontext}{\pc}{E[e']}{\tau}$ (\todo{???})

          \item[Case W-App:] Given $e = {(\where{v}{\delexp{p}{q}})~v'}$ and 
		  
		  $e' = \where{(v~v')}{\delexp{p}{q}}$. We have to prove that 
		\[
		\fexp{\delegcontext}{\varcontext}{\pc}{\where{(v~v')}{\delexp{p}{q}}}{\tau}
		\]
        From \ruleref{App} we have: 
                \begin{align}
		\fexpPGTpc{\where{v}{\delexp{p}{q}}}{\func{τ_1}{\pc'}{τ}}\label{eq:subwapp1}  \\
                 \fexpPGTpc{v'}{τ₁}\label{eq:subwapp2} \\
                \rflowjudge{\Pi;\pubtrust;\pc'}{\pc}{\pc'} \label{eq:subwapp3}
                \end{align}
                Rule \ruleref{Where} gives us the following:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:subwapp4}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:subwapp5} \\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:subwapp5}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\func{τ_1}{\pc'}{τ}} \label{eq:subwapp6}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:subwapp7}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:subwapp8}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\func{\tau_1}{\pc'}{\tau}} \label{eq:subwapp9}
                \end{align}
        We now want to show that $e'$ is well typed via \ruleref{Where}. The key premise is to show that the 
        subexpression $(v~v')$ is well-typed via \ruleref{App}. That is,
	\begin{equation}
		\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc }{v~v'}{τ} \label{eq:subwapp10}
	\end{equation}
	
	First, from \eqref{eq:subwapp2}, \eqref{eq:subwapp3}
	and Lemma~\ref{lemma:piweaken}:	
       \begin{align}
       \fexp{Π,\langle \aftypep{p}{q} \mid \pc \sqcup \ell \rangle}{\varcontext}{\pc}{v'}{τ₁} \\
	       \rflowjudge{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell} ;\pubtrust;\pc'}{\pc}{\pc'} 
       \end{align}
       Combining with \eqref{eq:subwapp6}, we have \eqref{eq:subwapp10}. 
       From \eqref{eq:subwapp9} and \ruleref{P-Fun}, we have $\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau}$.
       Remaining clauses give us
		\[
		\fexp{\delegcontext}{\varcontext}{\pc}{\where{(v~v')}{\delexp{p}{q}}}{\tau}
		\]
         
          \item[Case W-TApp:] Given $e = {(\where{v}{\delexp{p}{q}})~\tau}$ and 
		  
		  $e' = \where{(v~\tau')}{\delexp{p}{q}}$. We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(v~\tau')}{\delexp{p}{q}}}{\tau[X \mapsto \tau']}
		\]
        From \ruleref{TApp} we have: 
                \begin{align}
		\fexpPGTpc{\where{v}{\delexp{p}{q}}}{\tfuncpc{X}{\pc'}{τ}}\label{eq:subwtapp1}  \\
                \rflowjudge{\Pi;\pubtrust;\pc'}{\pc}{\pc'} \label{eq:subwtapp2}
                \end{align}
                Rule \ruleref{Where} gives us the following:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:subwtapp4}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:subwtapp5} \\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:subwtapp5}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\tfuncpc{X}{\pc'}{τ}} \label{eq:subwtapp6}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:subwtapp7}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:subwtapp8}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\tfuncpc{X}{\pc'}{\tau}} \label{eq:subwtapp9}
                \end{align}
        We now want to show that $e'$ is well typed via \ruleref{Where}. The key premise is to show that the 
        subexpression $(v~\tau')$ is well-typed via \ruleref{TApp}. That is,
	\begin{equation}
		\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc }{v~\tau'}{τ[X \mapsto \tau']} \label{eq:subwtapp10}
	\end{equation}
	
	First, from \eqref{eq:subwtapp2}
	and weakening delegation context (Lemma~\ref{lemma:piweaken}), we get:	
       \begin{align}
	       \rflowjudge{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell} ;\pubtrust;\pc'}{\pc}{\pc'} 
       \end{align}
       Combining with \eqref{eq:subwtapp6}, we have \eqref{eq:subwtapp10}. 
       From \eqref{eq:subwtapp9} and \ruleref{P-TFun}, we have $\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau}$. Since type substitution preserves protection (Lemma ~\ref{lemma:substprot}), we have 
       $\protjudge{\delegcontext;\pubtrust;\ell'}{\pc}{\tau [ X \mapsto \tau']}$.
       Remaining clauses give us
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(v~\tau')}{\delexp{p}{q}}}{\tau [X \mapsto \tau']}
		\]
          \item[Case W-BindM:] 
			Given $e = {\bind{x}{(\where{v}{\delexp{p}{q}})}{e}}$ and $e' = {\where{(\bind{x}{v}{e})}{\delexp{p}{q}}}$. We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\bind{x}{v}{e})}{\delexp{p}{q}}}{\tau}
		\]
        From \ruleref{BindM} we have: 
                \begin{align}
			\fexpPGTpc{(\where{v}{\delexp{p}{q}})}{\says{\ell'''}{\tau'}} \label{eq:bind1} \\
			\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc \sqcup \ell''' \sqcup \ell''''}{e}{\tau} \label{eq:bind2} \\
			\rflowjudge{\delegcontext;\pubtrust; \ell''''}{\pc}{\ell''''} \label{eq:bind3}\\
			\protjudge{\delegcontext;\pubtrust; \ell''''}{\pc \sqcup \ell''' \sqcup \ell''''}{\tau} \label{eq:bind4}
	\end{align}

	From \eqref{eq:bind1} and rule \ruleref{Where}, we get the following:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:bind5}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:bind6}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:bind7}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\says{\ell'''}{\tau'}} \label{eq:bind8}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:bind9}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:bind10}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau} \label{eq:bind11}
                \end{align}
        We now want to show that $e'$ is well typed via \ruleref{Where}. That is, we need the following premises, 
	\begin{align}
		\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{\bind{x}{v}{e}}{\tau} \label{eq:bind12} \\
	       \fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:bind13}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:bind14}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:bind15}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:bind16}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:bind17}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\tau} \label{eq:bind18}
       \end{align}


       From \eqref{eq:bind8}, \eqref{eq:bind2}, \eqref{eq:bind3} and \eqref{eq:bind4}, we have
		\fexp{\delegcontext}{\varcontext}{\pc}{\bind{x}{v}{e}}{\tau}. Weakening the delegation context (Lemma~\ref{lemma:piweaken}), we have \eqref{eq:bind12}. 
      We already have \eqref{eq:bind13} from \eqref{eq:bind5}; \eqref{eq:bind14} from \eqref{eq:bind6}; \eqref{eq:bind15} from \eqref{eq:bind7}; \eqref{eq:bind16} from \eqref{eq:bind9}; \eqref{eq:bind17} from \eqref{eq:bind10} and \eqref{eq:bind18} from \eqref{eq:bind11}.

       Combining, we have 
       \[
		\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\bind{x}{v}{e})}{\delexp{p}{q}}}{\tau}
	\]
        
          \item[Case W-Assume:] 
			Given $e = {\assume{(\where{v}{\delexp{p}{q}})}{e}}$ and $e' = {\where{(\assume{v}{e})}{\delexp{p}{q}}}$. We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\assume{v}{e})}{\delexp{p}{q}}}{\tau}
		\]
        From \ruleref{Assume} we have: 
                \begin{align}
			\fexpPGTpc{\where{v}{\delexp{p}{q}}}{\aftype{a}{b}} \label{eq:assume1}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:assume2} \\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:assume3} \\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau} \label{eq:assume4}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:assume5} \\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:assume6}\\
			\fexp{\delegcontext, \delexpl{a}{b}{\pc \sqcup \ell}}{\varcontext}{\pc \sqcup \ell \sqcup \ell'}{e}{\tau} \label{eq:assume7}
		\end{align}
	From \eqref{eq:assume1} and rule \ruleref{Where}, we get the following:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:assume8}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:assume9}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:assume10}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\aftype{a}{b}} \label{eq:assume11}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:assume12}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:assume13}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau} \label{eq:assume14}
                \end{align}
		The key premise is to show that
		\begin{equation}
			\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{(\assume{v}{e})}{\tau}
		\end{equation}
		which follows from weakening delegation context (Lemma~\ref{lemma:piweaken}) in equations \eqref{eq:assume2} to \eqref{eq:assume5} and \eqref{eq:assume11}.
		Combining with other premises, we have
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\assume{v}{e})}{\delexp{p}{q}}}{\tau}
		\]

		\item[Case W-UnPair:] .
			Given $$e = {\proj{i}{(\where{\pair{v_1}{v_2}}{\delexp{p}{q}})}}$$ and $$e' = {\where{(\proj{i}{\pair{v_1}{v_2}})}{\delexp{p}{q}}}$$.
We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\proj{i}{\pair{v_1}{v_2}})}{\delexp{p}{q}}}{\tau_i}
		\]
		From \ruleref{UnPair}, we have:
		\begin{align}
			\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc}{\where{\pair{v_1}{v_2}}{\delexp{p}{q}}}{\prodtype{τ_1}{τ_2}} \label{eq:wunpair1} 
		\end{align}
		From \eqref{eq:wunpair1} and \ruleref{Where}, we have:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:wunpair2}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:wunpair3}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:wunpair4}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{\pair{v_1}{v_2}}{\prodtype{\tau_1}{\tau_2}} \label{eq:wunpair5}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:wunpair6}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:wunpair7}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\prodtype{\tau_1}{\tau_2}} \label{eq:wunpair8}
                \end{align}
		From \eqref{eq:wunpair5} and \ruleref{UnPair}, we have:
			\fexp{\delegcontext, \delexp{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{\proj{i}{\pair{v_1}{v_2}}}{\tau_i}

			From \eqref{eq:wunpair8} and \ruleref{P-Pair}, we have
			$
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau_i}$. 
		Combining with remaining premises (\eqref{eq:unpair2} to \eqref{eq:unpair7}) we have
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{\proj{i}{\pair{v_1}{v_2}}}{\delexp{p}{q}}}{\tau_i}

		\item[Case W-Case:]
			Given $$e = {\casexp{(\where{v}{\delexp{p}{q}})}{x}{e_1}{e_2}}$$ and $$e' = {\where{(\casexp{v}{x}{e_1}{e_2})}{\delexp{p}{q}}}$$.
We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\casexp{v}{x}{e_1}{e_2})}{\delexp{p}{q}}}{\tau}
		\]
        From \ruleref{Case} we have: 
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{v}{\delexp{p}{q}}}{τ_1 + τ_2} \label{eq:case1} \\
			\protjudge{\delegcontext;\pubtrust;\ell}{\pc \sqcup \ell}{\tau} \label{eq:case2} \\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{\pc}{\ell} \label{eq:case3} \\
			\fexp{\delegcontext}{\varcontext,~x:τ_1}{\pc \sqcup \ell }{e_1}{τ} \label{eq:case4} \\
			\fexp{\delegcontext}{\varcontext,~x:τ_2}{\pc \sqcup \ell}{e_2}{τ} \label{eq:case5} 
		\end{align}
	From \eqref{eq:case1} and rule \ruleref{Where}, we get the following:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:case6}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:case7}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:case8}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\sumtype{\tau_1}{\tau_2}} \label{eq:case9}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:case10}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:case11}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau} \label{eq:case12}
                \end{align}
		The key premise to prove is that:
		\[
			\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{(\casexp{v}{x}{e_1}{e_2})}{\tau}
		\]
		which follows from \eqref{eq:case9} and weakening delegations in equations \eqref{eq:case2} to \eqref{eq:case5}.
		Combining with remaining premises, we have
		$$\fexp{\delegcontext}{\varcontext}{\pc}{\where{(\casexp{v}{x}{e_1}{e_2})}{\delexp{p}{q}}}{\tau}$$.

		\item[Case W-UnitM:]
			Given $e = \return{\ell}{(\where{v}{\delexp{p}{q}})}$ and $e' = {\where{(\return{\ell}{v})}{\delexp{p}{q}}}$. We have to prove that 
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{\return{\ell}{v}}{\delexp{p}{q}}}{\says{\ell}{\tau}}
		\]
        From \ruleref{UnitM} we have: 
                \begin{align}
			\fexpPGTpc{\where{v}{\delexp{p}{q}}}{\tau} \label{eq:unit1}
	\end{align}
	From \ruleref{Where}, we have:
                \begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\delexp{p}{q}}{\aftype{p}{q}} \label{eq:unit1}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{q}} \label{eq:unit2}\\
			\rafjudge{\delegcontext;\pubtrust;\ell}{\voice{\confid{p}}}{\voice{\confid{q}}} \label{eq:unit3}\\
			\texp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{v}{\tau} \label{eq:unit4}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell}{\pc}{\ell} \label{eq:unit5}\\
			\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:unit6}\\
			\protjudge{\delegcontext;\pubtrust; \ell'}{\pc }{\tau} \label{eq:unit7}
                \end{align}

		From \eqref{eq:unit4} and \ruleref{UnitM}, we have
		\[
			\fexp{\delegcontext, \delexpl{p}{q}{\pc \sqcup \ell}}{\varcontext}{\pc}{\return{\ell}{v}}{\says{\ell}{\tau}}
		\]

		Combining with other premises (\eqref{eq:unit1} to \eqref{eq:unit7}), we have
			\fexp{\delegcontext}{\varcontext}{\pc}{\where{\return{\ell}{v}}{\delexp{p}{q}}}{\says{\ell}{\tau}}.

	\item[Case B-Step:] 
		Given $e  = \bracket{e_1}{e_2}$ and $e' = \bracket{e'_1}{e'_2}$. Also $\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1}{e_2}}{\tau}$. 
		We have to prove
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{{e'}_1}{{e'}_2}}{\tau} 
		\]
		Without loss of generality, let $i = 1$. Thus from the premises of \ruleref{B-Step}, we have $e_1 \stepsone {e'}_1$ and $ {e'}_2 = e_2$.
		From \ruleref{Bracket}, we have
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc'}{e_1}{\tau} \label{eq:bracket1}\\
			\fexp{\delegcontext}{\varcontext}{\pc'}{e_2}{\tau} \label{eq:bracket2}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\ell \sqcup \ell' \sqcup H^\pi \sqcup \pc)}{{\pc'}} \label{eq:bracket3}\\
			\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\tau} \label{eq:bracket4}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \label{eq:bracket5}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} \label{eq:bracket6} 
		\end{align}
		Since \eqref{eq:bracket1} holds, applying induction to the premise $e_1 \stepsone e'_1`$, we have that
			$\fexp{\delegcontext}{\varcontext}{\pc'}{e'_1}{\tau}$. 
			Combining with remaining premises (\eqref{eq:bracket2} to \eqref{eq:bracket6}) we thus have that
			$\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e'_1}{e'_2}}{\tau}$. 
	\item[Case B-App:] 
		Given $e  = \bracket{\lamc{x}{\tau_1}{\pc''}{e_1}}{\lamc{x}{\tau_1}{\pc''}{e_2}}~v $ and 
		$e' = \bracket{e_1~\outproj{v}{1}}{e_2~\outproj{v}{2}}$. 
		
		Also $\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\lamc{x}{\tau_1}{\pc''}{e_1}}{\lamc{x}{\tau_1}{\pc''}{e_2}}~v}{\tau_2}$. 
		We have to prove
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1[x \mapsto \outproj{v}{1}]}{e_2[ x \mapsto \outproj{v}{2}}]}{\tau_2} 
		\]
		That is, we need the following premises:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{e_i[x \mapsto \outproj{v}{i}]}{\tau_2} \label{eq:bapp11}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\hat{\ell} \sqcup \bar{\ell} \sqcup H^\pi \sqcup \pc)}{\hat{\pc}} \label{eq:bapp12}\\
			\protjudge{\delegcontext; \pubtrust; \bar{\ell}}{\hat{\pc}}{\tau_2} \label{eq:bapp14}\\
			\rflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\pc}{\hat{\ell}} \label{eq:bapp15}\\
			\rflowjudge{\delegcontext; \pubtrust; \bar{\ell}}{\pc}{\bar{\ell}} \label{eq:bapp16} 
		\end{align}	
From $\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\lamc{x}{\tau_1}{\pc''}{e_1}}{\lamc{x}{\tau_1}{\pc''}{e_2}}~v}{\tau_2}$
and \ruleref{App}, we have:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\lamc{x}{\tau_1}{\pc''}{e_1}}{\lamc{x}{\tau_1}{\pc''}{e_2}}}{\func{\tau_1}{\pc''}{\tau_2}} \label{eq:bapp1}\\
			\fexp{\delegcontext}{\varcontext}{\pc}{v}{\tau_1} \label{eq:bapp2}\\
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc}{\pc''} \label{eq:bapp3}
		\end{align}

		From \ruleref{Bracket} and \eqref{eq:bapp1}, we have
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc'}{\lamc{x}{\tau_1}{\pc''}{e_1}}{\func{\tau_1}{\pc''}{\tau_2}} \label{eq:bapp4}\\
			\fexp{\delegcontext}{\varcontext}{\pc'}{\lamc{x}{\tau_1}{\pc''}{e_2}}{\func{\tau_1}{\pc''}{\tau_2}} \label{eq:bapp5}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\ell \sqcup \ell' \sqcup H^\pi \sqcup \pc)}{\pc'} \label{eq:bapp6}\\
			\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\func{\tau_1}{\pc''}{\tau_2}} \label{eq:bapp8}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \label{eq:bapp9}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} \label{eq:bapp10} 
		\end{align}	

		Applying Lemma~\ref{lemma:proj} to \eqref{eq:bapp2}, we have 
		$\fexp{\delegcontext}{\varcontext}{\pc}{\outproj{v}{i}}{\tau_1}$ for $i = \{1,2\}$.

		Let $\hat{\pc} = \pc'$, $\hat{\ell} = \ell$ and $\bar{\ell} = \ell'$.
		From \eqref{eq:bapp8} and \ruleref{P-Fun}, we have
		\begin{align}
			\protjudge{\delegcontext; \pubtrust;\ell'}{\pc'}{\tau_2} \label{eq:bapp15} \\
			\rflowjudge{\delegcontext;\pubtrust;\ell'}{\pc'}{\pc''}\label{eq:bapp16} \\
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\ell'}{\pc''}\label{eq:bapp17} 
		\end{align}

		\eqref{eq:bapp15} is same as \eqref{eq:bapp14}. Using \ruleref{R-Weaken} on \eqref{eq:bapp16} and \eqref{eq:bapp17} we have
		\begin{equation}
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}\label{eq:bapp18} 
		\end{equation}

		From \eqref{eq:bapp4} and \ruleref{Lam}, we have
			$\fexp{\delegcontext}{\varcontext, x:\tau_1}{\pc''}{e_1}{\tau_2}$ and 
		applying Lemma~\ref{lemma:subst} we have
			$\fexp{\delegcontext}{\varcontext}{\pc''}{e_1[x \mapsto \outproj{v}{1}]}{\tau_2}$.
			Applying PC reduction (Lemma~\ref{lemma:pcred}) using \eqref{eq:bapp18}, we have \eqref{eq:bapp11}. 
		
		From \eqref{eq:bapp6}, \eqref{eq:bapp9} and \eqref{eq:bapp10} we have \eqref{eq:bapp12}, \eqref{eq:bapp14} and \eqref{eq:bapp15} respectively. Thus we have all the premises to prove:
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1[x \mapsto \outproj{v}{1}]}{e_2[ x \mapsto \outproj{v}{2}}]}{\tau_2} 
		\]

	\item[Case B-TApp:] 
		Given $e  = \bracket{\tlam{X}{\pc''}{e_1}}{\tlam{X}{\pc''}{e_2}}~\tau' $ and 
		$e' = \bracket{e_1~\tau'}{e_2~\tau'}$. 
		Also 
		
		$\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\tlam{X}{\pc''}{e_1}}{\tlam{X}{\pc''}{e_2}}~\tau'}{\tau}$. 
		We have to prove that
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1[x \mapsto \tau']}{e_2[ x \mapsto \tau'}]}{\tau[ X \mapsto \tau']} 
		\]
		That is, we need the following premises:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{e_i[X \mapsto \tau]}{\tau[X \mapsto \tau']} \label{eq:btapp11}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\hat{\ell} \sqcup \bar{\ell} \sqcup H^\pi \sqcup \pc)}{\hat{\pc}} \label{eq:btapp12}\\
			\protjudge{\delegcontext; \pubtrust; \bar{\ell}}{\hat{\pc}}{\tau[X \mapsto \tau']} \label{eq:btapp14}\\
			\rflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\pc}{\hat{\ell}} \label{eq:btapp15}\\
			\rflowjudge{\delegcontext; \pubtrust; \bar{\ell}}{\pc}{\bar{\ell}} \label{eq:btapp16} 
		\end{align}	
From $\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\tlam{X}{\pc''}{e_1}}{\tlam{X}{\pc''}{e_2}}~\tau'}{\tau}$
and \ruleref{TApp}, we have:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\tlam{X}{\pc''}{e_1}}{\tlam{X}{\pc''}{e_2}}}{\tfuncpc{X}{\pc''}{\tau}} \label{eq:btapp1}\\
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc}{\pc''} \label{eq:btapp3}
		\end{align}

		From \ruleref{Bracket} and \eqref{eq:btapp1}, we have
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc'}{\tlam{X}{\pc''}{e_1}}{\tfuncpc{X}{\pc''}{\tau}} \label{eq:btapp4}\\
			\fexp{\delegcontext}{\varcontext}{\pc'}{\tlam{X}{\pc''}{e_2}}{\tfuncpc{X}{\pc''}{\tau}} \label{eq:btapp5}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\ell \sqcup \ell' \sqcup H^\pi \sqcup \pc)}{\pc'} \label{eq:btapp6}\\
			\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\tfuncpc{X}{\pc''}{\tau}} \label{eq:btapp8}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \label{eq:btapp9}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} \label{eq:btapp10} 
		\end{align}	

		Let $\hat{\pc} = \pc'$, $\hat{\ell} = \ell$ and $\bar{\ell} = \ell'$.
		From \eqref{eq:btapp8} and \ruleref{P-Fun}, we have
		\begin{align}
			\protjudge{\delegcontext; \pubtrust;\ell'}{\pc'}{\tau_2} \label{eq:btapp15} \\
			\rflowjudge{\delegcontext;\pubtrust;\ell'}{\pc'}{\pc''}\label{eq:btapp16} \\
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\ell'}{\pc''}\label{eq:btapp17} 
		\end{align}

		\eqref{eq:btapp15} is same as \eqref{eq:btapp14}. Using \ruleref{R-Weaken} on \eqref{eq:btapp16} and \eqref{eq:btapp17} we have
		\begin{equation}
			\rflowjudge{\delegcontext;\pubtrust;\pc''}{\pc'}{\pc''}\label{eq:btapp18} 
		\end{equation}

		From \eqref{eq:btapp4} and \ruleref{TLam}, we have
			$\fexp{\delegcontext}{\varcontext, X}{\pc''}{e_1}{\tau}$ and 
		applying type substitution (Lemma~\ref{lemma:typesubst}) we have
			$\fexp{\delegcontext}{\varcontext}{\pc''}{e_1[X \mapsto \tau']}{\tau[ X \mapsto \tau']}$.
			Applying PC reduction (Lemma~\ref{lemma:pcred}) using \eqref{eq:btapp17}, we have \eqref{eq:btapp11}. 
		
		From \eqref{eq:btapp6}, \eqref{eq:btapp9} and \eqref{eq:btapp10} we have \eqref{eq:btapp12}, \eqref{eq:btapp14} and \eqref{eq:btapp15} respectively. Thus we have all the premises to prove:
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{e_1[X \mapsto \tau']}{e_2[ X \mapsto \tau'}]}{\tau[X \mapsto \tau']} 
		\]

	\item[Case B-UnPair:] 
		Given $e =\proj{i}{\bracket{\pair{v_{11}}{v_{12}}}{\pair{v_{21}}{v_{22}}}}$ and $e'  = \bracket{v_{1i}}{v_{2i}} $ 
		Also 
			\fexp{\delegcontext}{\varcontext}{\pc}{\proj{i}{\bracket{\pair{v_{11}}{v_{12}}}{\pair{v_{21}}{v_{22}}}}}{\tau_i} 
		We have to prove
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{v_{1i}}{v_{2i}}}{\tau_i} 
		\]
		From \ruleref{UnPair}, we have:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\pair{v_{11}}{v_{12}}}{\pair{v_{21}}{v_{22}}}}{\prodtype{\tau_1}{\tau_2}} \label{eq:bunpair1}
		\end{align}

		From \ruleref{Bracket}, we have
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc'}{\pair{v_{11}}{v_{12}}}{\prodtype{\tau_1}{\tau_2}} \label{eq:bunpair2}\\
			\fexp{\delegcontext}{\varcontext}{\pc'}{\pair{v_{21}}{v_{22}}}{\prodtype{\tau_1}{\tau_2}} \label{eq:bunpair3}\\
			\rflowjudge{\delegcontext;\pubtrust;\ell}{(\ell \sqcup \ell' \sqcup H^\pi \sqcup \pc)}{{\pc'}} \label{eq:bunpair4}\\
			\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\prodtype{\tau_1}{\tau_2}} \label{eq:bunpair5}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell}{\pc}{\ell} \label{eq:bunpair6}\\
			\rflowjudge{\delegcontext; \pubtrust; \ell'}{\pc}{\ell'} \label{eq:bunpair7} 
		\end{align}	
		From \eqref{eq:bunpair2}, \eqref{eq:bunpair3} and \ruleref{UnPair}, we have
			$\fexp{\delegcontext}{\varcontext}{\pc'}{v_{1i}}{\tau_i}$ and $\fexp{\delegcontext}{\varcontext}{\pc'}{v_{2i}}{\tau_i}$  for $i = \{1, 2\}$. 
			
			From \eqref{eq:bunpair5} and \ruleref{P-Pair}, we have
		$\protjudge{\delegcontext; \pubtrust; \ell'}{\pc'}{\tau_i}$.
		Combining with other premises, we have
	$		\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{v_{1i}}{v_{2i}}}{\tau_i}$. 
	\item[Case B-BindM1:] Invalid case as the given bracket expression isn't well-typed. 
	\item[Case B-Bind:] 
		Given $e = {\bind{x}{\bracket{\return{\ell}{v_1}}{\return{\ell}{v_2}}}{e}}$.
		Here $e' = {e[x \mapsto \bracket{v_1}{v_2}]}$  or 
		$e' = {\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}[x \mapsto {v_2}]}}$. 
		In either case, $\outproj{e[x \mapsto \bracket{v_1}{v_2}]}{i} = \outproj{\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}[x \mapsto {v_2}]}}{i}$.
		Also $\fexp{\delegcontext}{\varcontext}{\pc}{\bind{x}{\bracket{\return{\ell_1}{v_1}}{\return{\ell_2}{v_2}}}{e}}{\tau}$. 
		From \ruleref{BindM}, we have
		\begin{align}
			\fexpPGTpc{\bracket{\return{\ell}{v_1}}{\return{\ell}{v_2}}}{\says{\ell}{\tau'}} \label{eq:b1bindm1} \\
		\fexp{\delegcontext}{\varcontext, x:\tau'}{\pc \sqcup \ell \sqcup \ell'}{e}{\tau} \label{eq:b1bindm2} \\
		\rflowjudge{\delegcontext;\pubtrust; \ell'}{\pc}{\ell'} \label{eq:b1bindm3} \\
		\protjudge{\delegcontext;\pubtrust; \ell'}{\pc \sqcup \ell \sqcup \ell'}{\tau} \label{eq:b1bindm4} 
		\end{align}

		From \eqref{eq:b1bindm1} and \ruleref{Bracket}, we have
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\pc'}{\return{\ell}{v_1}}{\says{\ell}{\tau'}} \label{eq:b1bracket1}\\
		\fexp{\delegcontext}{\varcontext}{\pc'}{\return{\ell}{v_2}}{\says{\ell}{\tau'}} \label{eq:b1bracket2}\\
	\rflowjudge{\delegcontext;\pubtrust;\ell''}{(\ell'' \sqcup \ell''' \sqcup H^\pi \sqcup \pc)}{{\pc'}} \label{eq:b1bracket3}\\
			\protjudge{\delegcontext; \pubtrust; \ell'''}{\pc'}{\says{\ell}{\tau'}} \label{eq:b1bracket4}\\
		\rflowjudge{\delegcontext; \pubtrust; \ell''}{\pc}{\ell''} \label{eq:b1bracket5}\\
		\rflowjudge{\delegcontext; \pubtrust; \ell'''}{\pc}{\ell'''} \label{eq:b1bracket6} 
		\end{align}
		From \eqref{eq:b1bracket4}, we have that either 
		$\protjudge{\delegcontext; \pubtrust; \ell'''}{\pc'}{\tau'}$ (\ruleref{P-Lbl1}) or
		\rflowjudge{\delegcontext;\pubtrust;\ell'''}{\pc'}{\ell} (\ruleref{P-Lbl2}.
		If the former holds, then $e$ takes a non-deterministic step using \ruleref{B-BindM2} and if the latter holds, $e$ takes a non-deterministic step using \ruleref{B-BindM3}. 

		\begin{description}
	\item[Case B-BindM2:] 
		We have to prove that,
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{e[x \mapsto \bracket{v_1}{v_2}]}{\tau}	
		\]

		That is,
		\begin{align}
			\fexp{\delegcontext}{\varcontext, x: \tau'}{\pc}{e}{\tau} \label{eq:b2bindm1}\\	
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{v_1}{v_2}}{\tau'} \label{eq:b2bindm2}	
		\end{align}

		Since $\rflowjudge{\delegcontext;\pubtrust; \pc \sqcup \ell \sqcup \ell'}{\pc}{\pc \sqcup \ell \sqcup \ell'}$, applying PC reduction (Lemma~\ref{lemma:pcred}) to \eqref{eq:b1bindm2} we get \eqref{eq:b2bindm1}.

		For some $\hat{\pc}$, $\hat{\ell}$ and $\bar{\ell}$, we need the following premises to satisfy \ruleref{Bracket}:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{v_i}{\tau} \label{eq:b2bracket8}\\
			\rflowjudge{\delegcontext;\pubtrust; \hat{\ell}}{(\hat{\ell} \sqcup \bar{\ell} \sqcup H^\pi \sqcup \pc)}{{\hat{\pc}}} \label{eq:b2bracket10}\\
			\protjudge{\delegcontext; \pubtrust; \bar{\ell}}{\hat{\pc}}{\tau'} \label{eq:b2bracket11}\\
			\rflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\pc}{\hat{\ell}} \label{eq:b2bracket12}\\
			\rflowjudge{\delegcontext; \pubtrust; \bar{\ell}}{\pc}{\bar{\ell}} \label{eq:b2bracket13} 
		\end{align}

				Let $\hat{pc} = \pc'$, $\hat{\ell} = \ell''$ and $\bar{\ell} = \ell'''$. From \eqref{eq:b1bracket4}, we have $\protjudge{\delegcontext;\pubtrust;\ell'''}{\pc'}{\tau'}$ (from assumption) and so we have \eqref{eq:b2bracket11}. Other premises follow from \eqref{eq:b1bracket3}, \eqref{eq:b1bracket5} and \eqref{eq:b1bracket6}.
		Thus
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}[x \mapsto {v_2}]}}{\tau}	
		\]
	\item[Case B-BindM3:] 
		We have to prove that
		\[
			\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}[x \mapsto {v_2}]}}{\tau}	
		\]
		For some $\hat{\pc}$, $\hat{\ell}$ and $\bar{\ell}$, we need the following premises to satisfy \ruleref{Bracket}:
		\begin{align}
			\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{e [x \mapsto v_1]}{\tau} \label{eq:b1bracket8}\\
			\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{e [ x \mapsto v_2]}{\tau} \label{eq:b1bracket9}\\
			\rflowjudge{\delegcontext;\pubtrust; \hat{\ell}}{(\hat{\ell} \sqcup \bar{\ell} \sqcup H^\pi \sqcup \pc)}{{\hat{\pc}}} \label{eq:b1bracket10}\\
			\protjudge{\delegcontext; \pubtrust; \bar{\ell}}{\hat{\pc}}{\tau} \label{eq:b1bracket11}\\
			\rflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\pc}{\hat{\ell}} \label{eq:b1bracket12}\\
			\rflowjudge{\delegcontext; \pubtrust; \bar{\ell}}{\pc}{\bar{\ell}} \label{eq:b1bracket13} 
		\end{align}

		Let $\hat{pc} = \pc \sqcup \ell \sqcup \ell'$, $\bar{\ell} = \ell'$ and $\hat{\ell} = \ell'' \sqcup \ell''' $.
	
	\medskip
		From \eqref{eq:b1bindm2}, Lemma~\ref{lemma:proj} and Lemma~\ref{lemma:subst}, we have \eqref{eq:b1bracket8} and \eqref{eq:b1bracket9}.
		From \eqref{eq:b1bindm4} and \eqref{eq:b1bindm3} we have \eqref{eq:b1bracket11} and \eqref{eq:b1bracket13} respectively.
				From \eqref{eq:b1bracket4} and \ruleref{P-Lbl1}, we have $\rflowjudge{\delegcontext;\pubtrust;\ell'''}{\pc'}{\ell}$ and so by \ruleref{R-Weaken} we have $\rflowjudge{\delegcontext;\pubtrust; \ell'' \sqcup \ell'''}{\pc'}{\ell}$ (from assumption). 

	\medskip
		From \eqref{eq:b1bracket3} and \ruleref{R-Weaken}, we have
	$\rflowjudge{\delegcontext;\pubtrust;\ell'' \sqcup \ell'''}{(\ell'' \sqcup \ell''' \sqcup H^\pi \sqcup \pc)}{{\pc'}}$ and so $\rflowjudge{\delegcontext;\pubtrust;\ell'' \sqcup \ell'''}{(\ell'' \sqcup \ell''' \sqcup H^\pi)}{{\pc'}}$.
	From Lemma~\ref{lemma:flowtrans}, we have 
\[	
	\rflowjudge{\delegcontext;\pubtrust;\ell'' \sqcup \ell'''}{(\ell'' \sqcup \ell''' \sqcup H^\pi)}{{\pc \sqcup \ell \sqcup \ell'}}
\]
	We already have that 
	\[
		\rflowjudge{\delegcontext;\pubtrust;\ell'' \sqcup \ell'''}{(\ell' \sqcup \pc )}{{\pc \sqcup \ell \sqcup \ell'}}
	\]

	Combining both we have \eqref{eq:b1bracket10}.
	From \eqref{eq:b1bracket5}, \eqref{eq:b1bracket6} and \ruleref{R-Weaken} we have \eqref{eq:b1bracket13}. Thus we have all premises necessary to prove
			$\fexp{\delegcontext}{\varcontext}{\pc}{\bracket{\outproj{e}{1}[x \mapsto {v_1}]}{\outproj{e}{2}[x \mapsto {v_2}]}}{\tau}$.	
	\end{description}
	\item[Case B-Case:] Invalid case as the given bracket expression isn't well-typed. 
\end{description}
\end{proof}

\begin{lemma}[Delegation Invariance Lemma] \label{lemma:di}
	 Let \fexp{\delegcontext}{\varcontext}{\pc}{e}{\tau} such that $e \stepsto \where{e'}{v}$ and \lpre be the upper bound on all result labels in \delegcontext. Then the following hold:
	 \begin{enumerate}
		 \item There exist $r,t \in \L$ and $\delegcontext' = \delegcontext, \delexpl{r^\pi}{t^\pi}{\pc \sqcup \ell}$ such that  $\fexp{\delegcontext}{\varcontext}{\pc}{v}{\aftype{r^\pi}{t^\pi}}$, $\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{t^{\pi}}}$ and
\fexp{\delegcontext'}{\varcontext}{\pc}{e'}{\tau}.
		\item
		For all principals $p$ and $q$,
			 if $\notrafjudge{\delegcontext; \pubtrust; \lpre}{p^{\pi}}{q^{\pi}}$ and $\notrafjudge{\delegcontext;\pubtrust;\lpre}{\pc}{\voice{{q^\pi} - {p^\pi}}}$, 
	then
	\[
		\notrafjudge{\delegcontext';\pubtrust;\lpost}{p^\pi}{q^\pi}
	\]
	where
	\[
		\lpost = \begin{cases} \lpre &\mbox{ if } \pc \sqcup \ell \sqsubseteq \lpre \\
			\pc \sqcup \ell &\mbox{ if } \lpre \sqsubseteq \pc \sqcup \ell \\
			\pc \sqcup \ell \sqcup \lpre &\mbox{ otherwise }
		\end{cases}
	\]
	\end{enumerate}
\end{lemma}
\begin{proof}
Using subject reduction (Lemma~\ref{lemma:subred}), we have
\fexp{\delegcontext}{\varcontext}{\pc}{\where{e'}{v}}{\tau}. 
From \ruleref{Where} we have
\fexp{\delegcontext'}{\varcontext}{\pc}{e'}{\tau}.

\medskip

We prove the second part by contradiction. Assume that
	\begin{equation}
		\rafjudge{\delegcontext';\pubtrust;\lpost}{p^\pi}{q^\pi} \label{eq:di1}
	\end{equation}
Let $(p^\pi, q_s, q_d)$ be the minimal $(\delegcontext;\lpre)$-factorization of $(p^\pi, q^\pi)$. So,
	\[ 
	\rafjudge{\delegcontext;\pubtrust;\lpre}{p^\pi}{q_s}
	\]
Since $\notrafjudge{\delegcontext; \pubtrust; \lpre}{p^{\pi}}{q^{\pi}}$, this implies that 
	\begin{align}
		\notrafjudge{\delegcontext;\pubtrust;\lpre}{p^\pi}{q_d} \label{eq:di2}
	\end{align}
	From \eqref{eq:di1}, we have that
	\begin{equation}
		\rafjudge{\delegcontext';\pubtrust;\lpost}{p^\pi}{q_d} \label{eq:di3}
	\end{equation}
	\emph{Since \lpre is an upper bound on the result labels in $\delegcontext$, notice that changing the result label \lpre in \eqref{eq:di2} to \lpost does not induce more trust relationships.} 
	So any derivation of \eqref{eq:di3} involves the derivation of
	$\rafjudge{\delegcontext'; \pubtrust; \lpre}{r^\pi}{t^\pi}$ via \ruleref{R-Assume}. 
	
	From \eqref{eq:di2} and \eqref{eq:di3} we have that either $\rafjudge{\delegcontext;\pubtrust; \lpre}{t^\pi}{q_d}$ or $\notrafjudge{\delegcontext;\pubtrust;\lpre}{t^\pi}{q_d}$. 
	This is because \eqref{eq:di3} is only possible because of the additional delegation $\delexp{r^\pi}{t^\pi}$ and so $t^\pi$ must enable a trust relation from $q_d$ to $p$. This can be done in two ways: either $t^\pi$ can act on behalf of full $q_d$ or act on behalf of a partial $q_d$.
	If the latter holds, then $\rafjudge{\delegcontext;\pubtrust;\lpre}{t^\pi}{q_1}$ such that $ q_d \equiv q_1 \wedge q_2$ and $\notrafjudge{\delegcontext;\pubtrust;\lpre}{t^\pi}{q_2}$. 
	So $\rafjudge{\delegcontext;\pubtrust;\lpre}{p^\pi}{q_s \wedge q_2}$ should hold as $t^\pi$ doesn't induce any additional trust flows from $q_2$.
	This implies that $(p, q_s \wedge q_2, q_1)$ is a $(\delegcontext-\lpre)$ factorization. Following the definition of minimal-factorization, we thus have that $\rafjudge{\delegcontext;\pubtrust; \lpre}{q_2}{q_d}$.
	From \ruleref{R-Trans}, we now have that $\rafjudge{\delegcontext; \pubtrust; \lpre}{t^\pi}{q_d}$ which is a contradiction stemming from the assumption $\notrafjudge{\delegcontext;\pubtrust;\lpre}{t^\pi}{q_d}$. Hence
	\begin{align}
		\rafjudge{\delegcontext; \pubtrust; \lpre}{t^\pi}{q_d} \label{eq:di8} \\
		\implies \rafjudge{\delegcontext; \pubtrust; \lpre}{\voice{t^\pi}}{\voice{q_d}} \label{eq:di9}
	\end{align}
	From \ruleref{Where}, we have that $\rafjudge{\delegcontext;\pubtrust;\ell}{\pc}{\voice{t^\pi}}$. Since $\ell \sqsubseteq \lpre$, weakening the result label (using \ruleref{R-Weaken}) gives 
	\begin{align}
		\rafjudge{\delegcontext; \pubtrust; \lpre}{\pc}{\voice{t^\pi}} \label{eq:di10}
	\end{align}
	Applying \ruleref{R-Trans} to \eqref{eq:di9} and \eqref{eq:di10} we have 
	$\rafjudge{\delegcontext;\pubtrust; \lpre}{\pc}{\voice{q_d}}$ contradicting the given fact 
$\notrafjudge{\delegcontext;\pubtrust;\lpre}{\pc}{\voice{{q^\pi} - {p^\pi}}}$.
	This is due to our assumption in \eqref{eq:di1} and so
	$$ \notrafjudge{\delegcontext; \pubtrust; \lpost}{p^\pi}{q^\pi}$$
\end{proof}
\begin{theorem}[FLAC Noninterference]
	Let \fexp{\delegcontext}{\varcontext,x:τ}{pc}{e}{\says{\ell}{bool}} and \lmax be the upper bound on the result label of all delegations in \delegcontext.
	If there exists some H such that:
	\begin{enumerate}
		\item \protjudge{\delegcontext; \pubtrust; \lmax }{H^{\pi}}{τ};
		\item $\notrflowjudge{\delegcontext;\pubtrust;\lmax}{H^{\pi}}{\ell^{\pi}}$;
		\item 
			\begin{enumerate}[label = (\alph*), ref=\theenumi{} (\alph*)]
				\item \label{3a} if $\pi = \rightarrow$ then \notrafjudge{\delegcontext;\pubtrust; \lmax}{\pc}{\voice{{\confid{H}} - {\confid{\ell}}}}
				\item \label{3b} if $\pi = \leftarrow $ then \notrafjudge{\delegcontext;\pubtrust; \lmax}{\pc}{(\integ{\ell} - \integ{H})}
			\end{enumerate}
	\end{enumerate}
	then for all $v_1, v_2$ with \texp{\delegcontext}{\varcontext}{\pc}{v_i}{s}, if $e[x \mapsto v_i] \rightarrow^{*} v'_i$, then $v'_1 = v'_2$.
\end{theorem}
\begin{proof}
	Let $e[x \mapsto \bracket{v_1}{v_2}] \stepsto v'$ such that $\outproj{v'}{i} = v'_i$ for $i = \{1, 2\}$.
	From subject reduction (Lemma~\ref{lemma:subred}) we have
	\fexp{\delegcontext}{\varcontext}{\pc}{v'}{\says{\ell}{"bool"}}.
	We have to prove that $\outproj{v'}{1} = \outproj{v'}{2}$. 

	\medskip
	Let us assume that $v'$ is a bracket value. Then by \ruleref{Bracket}, we have the following:
	\begin{align}
		\fexp{\delegcontext}{\varcontext}{\hat{\pc}}{\outproj{v'}{i}}{\says{\ell}{"bool"}} \label{eq:nibracket1}\\
			\rflowjudge{\delegcontext;\pubtrust; \hat{\ell}}{(\hat{\ell} \sqcup \bar{\ell} \sqcup H^\pi \sqcup \pc)}{{\hat{\pc}}} \label{eq:nibracket2}\\
			\protjudge{\delegcontext; \pubtrust; \bar{\ell}}{\hat{\pc}}{\says{\ell}{"bool"}} \label{eq:nibracket3}\\
			\rflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\pc}{\hat{\ell}} \label{eq:nibracket4}\\
			\rflowjudge{\delegcontext; \pubtrust; \bar{\ell}}{\pc}{\bar{\ell}} \label{eq:nibracket5} 
	\end{align}

	Since $\notrflowjudge{\delegcontext;\pubtrust;\lmax}{H^{\pi}}{\ell^{\pi}}$, we have that 
	\emph{$\notrflowjudge{\delegcontext;\pubtrust;\hat{\ell}}{H^{\pi}}{\ell^{\pi}}$ for any $\hat{\ell}$ since $\hat{\ell}$ is bounded from above by $\lmax$}. 
	Coupled with \eqref{eq:nibracket2}, we  have that $\notrflowjudge{\delegcontext; \pubtrust; \hat{\ell}}{\hat{\pc}}{\ell}$ for any $\hat{\ell}$ that is bounded from above by $\lmax$. Hence $\notprotjudge{\delegcontext;\pubtrust; \bar{\ell}}{\hat{\pc}}{\says{\ell}{"bool"}}$. Thus 
	\fexp{\delegcontext}{\varcontext}{\pc}{v'}{\says{\ell}{"bool"}} cannot be well-typed by \ruleref{Bracket} and so $v'$ itself isn't a bracket term.

	\medskip
	Note that $v'$ can only be a "where" term. We can prove this by inducting on the structure of the value. The only interesting case is $\return{\ell}{v''}$. In this case, we can easily prove that $v''$ cannot be a bracket term because sumtypes ("bool" = \sumtype{\voidtype}{\voidtype}) cannot protect any principal.

	Without loss of generality, let $v' = \where{w}{\delexp{p}{q}}$.
	We now need to prove that either $w$ is not a bracket term or that $\outproj{w}{1} = \outproj{w}{2}$.
	We prove this by induction on the number of "where" terms. For base case, where there are zero "where" terms, we already proved that $v'$ is not a bracket term. 
	For the induction step, we need to prove that 
	$v' = w~"where"~{\delexp{p}{q}}~"where"^n{\delexp{p_n}{q_n}}$ is not a bracket term. From induction hypothesis, we have that $w~"where"^n{\delexp{p_n}{q_n}}$ itself is not a bracket term. 

	\todo{Flesh out the inductive argument fully}.
	Thus it remains to prove that $w~"where"~{\delexp{p}{q}}$ is not a bracket term. 
	\begin{description}
		\item[Case $\pi = \rightarrow$:]
			From condition 2, we have $\notrflowjudge{\delegcontext;\pubtrust; \lmax}{\confid{H}}{\confid{\ell}}$. Invoking the delegation invariance (Lemma~\ref{lemma:di}) using condition ~\ref{3a}, we have that $\notrafjudge{\delegcontext';\pubtrust; \lpost}{\confid{\ell}}{\confid{H}}$ where $\delegcontext' = \delegcontext, \delexpl{p}{q}{\ell'}$ for some suitable $\ell'$ and $\lpost$ is the new upper bound on the result labels in $\delegcontext'$. 
			Note that this is same as $\notrflowjudge{\delegcontext';\pubtrust; \lpost}{\confid{H}}{\confid{\ell}}$. Running an argument similar to the base case, we have that $w$ cannot be a bracket term (as $\notprotjudge{\delegcontext;\pubtrust; \bar{\ell}}{\hat{\pc}}{\says{\ell}{"bool"}}$ for any $\bar{\ell}$).

		\item[Case $\pi = \leftarrow$:]
			Since $(\integ{\ell} - \integ{H})$ = $\voice{\integ{\ell} - \integ{H}}$ (\todo{Trivial?}), we have $\notrafjudge{\delegcontext;\pubtrust; \lmax}{\pc}{\voice{\integ{\ell} - \integ{H}}}$. Similar to above the above case, invoking Lemma~\ref{lemma:di} using ~\ref{3b}, we have 
			$\notrafjudge{\delegcontext';\pubtrust; \lpost}{\integ{H}}{\integ{\ell}}$ and so 
			$\notrflowjudge{\delegcontext';\pubtrust; \lpost}{\integ{H}}{\integ{\ell}}$. 
			Again $w$ cannot be a bracket term. 
	\end{description}
	This completes the proof that $v'$ isn't a bracket term and so $\outproj{v'}{1} = \outproj{v'}{2}$.
\end{proof}

